Zetta $\zeta$: An Efficient Closed-Loop Embodied Harness for Self-Evolving Physical Intelligence

Embodied agents are increasingly used to close the gap left by end-to-end policy models. Yet the agentic path has not realized closed-loop learning in physical execution: existing harnesses remain largely open-loop, following fixed skills during rollout and reflecting only after an episode completes. Such post-hoc reflection cannot govern execution as it unfolds, because physical interaction requires decisions to track rapidly changing robot-environment states at a frequency beyond today's large agentic models. We present Zetta, a closed-loop embodied harness that evolves code-based runtime critics and recovery skills online while keeping the base policy frozen. Through three timescale-separated loops, Zetta provides action-frequency governance, rollout-level critic-recovery proposal, and validation-gated skill updates. Together with Z-Infra, a rollout infrastructure decoupling agent logic from heterogeneous execution resources, Zetta achieves state-of-the-art success on LIBERO-Pro and RoboCasa under our current rollout budget, reaching 90.8% and 93.6%, with an 11.1x inference speedup; success continues to scale with self-exploration experience; learned skills transfer zero-shot, and clear robotic "Aha Moments" emerge. These results show that closed-loop harness self-evolution opens a scaling path for reliable physical intelligence.

==> arxiv_submission/tex/abstract.tex <==
\begin{abstract}
Embodied agents are increasingly used to close the gap left by end-to-end policy models. Yet the agentic path has not realized closed-loop learning in physical execution: existing harnesses remain largely open-loop, following fixed skills during rollout and reflecting only after an episode completes. Such post-hoc reflection cannot govern execution as it unfolds, because physical interaction requires decisions to track rapidly changing robot-environment states at a frequency beyond today’s large agentic models. We present \sys, a closed-loop embodied harness that evolves code-based runtime critics and recovery skills online while keeping the base policy frozen. Through three timescale-separated loops, Zetta provides action-frequency governance, rollout-level critic-recovery proposal, and validation-gated skill updates. Together with Z-Infra, a rollout infrastructure decoupling agent logic from heterogeneous execution resources, Zetta achieves state-of-the-art success on LIBERO-Pro and RoboCasa under our current rollout budget, reaching 90.8\% and 93.6\%, with a $11.1\times$ inference speedup; success continues to scale with self-exploration experience; learned skills transfer zero-shot, and clear robotic ``Aha Moments'' emerge. These results show that closed-loop harness self-evolution opens a scaling path for reliable physical intelligence.
% Embodied agents are increasingly used to close the gap left by end-to-end policy models.
% Yet existing embodied agent harnesses remain static and open-loop, following fixed skills rather than adapting to dynamic environments during rollout, because physical execution demands high-frequency governance that today's agentic reflection cannot provide. We present \sys, a closed-loop embodied harness that evolves code-based runtime critics and recovery skills online while the base policy model stays frozen. Three loops operate at different timescales to enable the harness self-evolution: a Critic-Governed Action Loop governs execution at action frequency, a Rollout-Batch Candidate Optimization Loop proposes candidate critics and recoveries from clustered failures, and a Validation-Gated Skill Update Loop admits only updates that improve and generalize success. We further build Z-Infra, the first rollout infrastructure designed for self-evolving embodied agents, decoupling agent logic from hardware. Evaluating on LIBERO and RoboCasa, \sys achieves state-of-the-art task success, continuously scales with evolution iterations, transfers learned skills zero-shot across tasks, and substantially increases rollout throughput, showing that harness self-evolution is a viable path toward reliable embodied intelligence.
\end{abstract}


==> arxiv_submission/tex/conclusion.tex <==
\section{Conclusion}
We presented \sys, a closed-loop embodied harness that closes the gap between static, open-loop agent harnesses and the high-frequency governance that physical execution demands, by evolving code-based runtime critics and recovery skills online while keeping the base policy model frozen. Through three coordinated loops operating at action, rollout-batch, and iteration timescales, \sys turns accumulated rollout experience into validated, generalizable improvements in execution behavior. To sustain this evolution, we built Z-Infra, the first rollout infrastructure designed for self-evolving embodied agents, decoupling agent logic from heterogeneous execution resources. Our experiments on LIBERO and RoboCasa show that this self-evolution scales task success toward the frozen policy's capability ceiling and transfers across tasks, demonstrating that harness self-evolution is a viable path toward reliable embodied intelligence.

Looking ahead, we plan to extend \sys and Z-Infra to real robots: enabling fast, massively parallel rollout collection and self-evolution directly for real machines by bridging the sim-to-real gap, and integrating real-robot environments as first-class workers within Z-Infra alongside simulated ones.

==> arxiv_submission/tex/experiment.tex <==
\newpage

\section{Experiments}


\subsection{Experimental Setup}
\label{sec:4_setup}

We evaluate the framework on LIBERO-Pro \cite{libero_pro} and RoboCasa \cite{nasiriany2024robocasa} benchmarks using a high-performance cluster equipped with \textbf{8 NVIDIA GeForce RTX 4090 GPUs}, enabling parallel rollouts and accelerated offline evolution.

For these experiments, we utilize specific pre-trained models as the underlying frozen base policies:
\begin{itemize}
    \item \textbf{LIBERO-Pro Benchmark}: Employs the $\pi_{0.5}$ \cite{black2025pi05} model as the base policy.
    \item \textbf{RoboCasa Benchmark}: Employs the GR00T N1.5 \cite{bjorck2025groot} model as the base policy.
\end{itemize}
Throughout all experiments, deployment-time evolution does not involve fine-tuning the weights of these base VLA models.

For both RoboCasa and LIBERO-Pro, we adhere to a \textbf{strict generalization evaluation protocol}: upon completion of the evolution, the final harness is evaluated on a \textbf{separate, strictly isolated set of test seeds} that were never seen by the Evolutionary Agent during the entire evolution and development process.

Specific implementation details for each benchmark are as follows:

\paragraph{RoboCasa: Random-Distribution Generalization.}
This evaluates the framework's generalization capabilities against challenging long-tail distributions, utilizing randomly sampled seeds for both development and testing.
\begin{enumerate}
    \item \textbf{Setup}: For each task, we randomly sample 50 environment seeds for development and evolution.
    \item \textbf{Evolutionary and Repair Cycle}: In each round, we collect failure trajectories from these 50 seeds and cluster them based on failure signatures. For each failure cluster, we select the representative medoid seed for diagnosis and repair development.
    \item \textbf{Final Evaluation (Held-Out)}: Upon completion, the final evaluation is conducted on a separate, strictly isolated set of 50 RoboCasa environment seeds (disjoint from the development set) to report the definitive success rate.
\end{enumerate}
\paragraph{LIBERO-Pro: Development-Test Generalization.}
This tests the framework's ability to generalize from a development set to entirely unseen task environments.
\begin{enumerate}
    \item \textbf{Setup}: For each task, we randomly sample 50 development seeds (Parent seeds, excluding seeds 1-20) for evolution.
    \item \textbf{Evolutionary Cycle and Repair}: Based on clustering of trajectories from the 50 development seeds, we target the erroneous seeds from the maximum failure cluster for repair development. Iteration continues until the success rate on these specific development seeds reaches $\ge 50\%$.
    \item \textbf{Final Evaluation (Held-Out)}: Upon completion, the final evaluation is conducted exclusively on the strictly isolated seeds 1 through 20 to report the SR.
\end{enumerate}




% \subsection{Physical Intelligence "Aha" Moments}

% To validate that Z-Harness enables discontinuous capability gains through physical intelligence rather than additional policy training, we analyze the fine-grained evolutionary trajectory within individual outer-loop cycles. We present \textbf{"Aha" moments}—instances where the system transitions from stagnant performance to high success rates by identifying and resolving the true physical bottleneck of a task.

% We define an "Aha" moment empirically by tracking success rates across \textbf{selected cumulative internal versions} within the evolution of a single failure cluster. These checkpoints represent intermediate refinements made by the Evolutionary Agent during offline diagnosis and repair, rather than separate outer-loop rollouts or additional VLA training. The base VLA policy remains frozen throughout.

% Through case studies on representative tasks from RoboCasa and LIBERO-Pro, we demonstrate that:
% \begin{enumerate}
% \item Early repairs often yield marginal gains or overfit specific failures, leading to performance plateaus.
% \item A true "Aha" moment occurs when the agent isolates the critical physical state variable (e.g., grasp retention, end-effector re-alignment, or pre-contact approach geometry) required for reliable VLA execution.
% \item Resolving this bottleneck produces a sharp, discontinuous increase in success rate, demonstrating that the harness acquires the necessary embodied intelligence to govern physical execution.
% \end{enumerate}



% \subsubsection{"Aha" Moments on Robocasa}
% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=0.95\textwidth]{figs/robocasa-results/fig_use/loop2_aha_moments.pdf}
%     \caption{\textbf{Physical-intelligence ``Aha'' moments within Loop-2
%     Stage-2 on Robocasa.} L2-v0 is the original Pure-VLA baseline, while L2-v1 is an
%     intermediate internal version after early critic and recovery revisions.
%     The flat L2-v0--L2-v1 segments summarize a period in which many candidate
%     fixes yield little robust improvement or overfit individual failures.
%     Once the agent identifies the task's key physical bottleneck and corrects
%     the associated critic and recovery mechanism, L2-v2 produces a sharp
%     success-rate increase. The plotted versions are selected internal
%     checkpoints, not outer-loop rollout rounds.}
%     \label{fig:robocasa-loop2-aha}
% \end{figure*}
% Figure~\ref{fig:robocasa-loop2-aha} shows this phenomenon on three
% representative RoboCasa tasks. We report task success rate at three selected
% checkpoints within Loop-2 Stage-2; these checkpoints are \emph{internal
% versions}, rather than separate outer-loop rollout rounds. L2-v0 is the
% original Pure-VLA baseline. L2-v1 is an intermediate state reached while the
% agent is still analyzing failures and repeatedly revising the critic and the
% recovery implementation, including its tool choice, parameters, and code.
% There can be many unshown repair attempts between the plotted checkpoints.
% Most early revisions produce only marginal gains or overfit the observed
% failures, so L2-v1 remains at the baseline success rate on all three tasks.

% An ``Aha'' moment occurs when a later internal version isolates the actual
% physical bottleneck and implements the corresponding critic and recovery
% mechanism. At L2-v2, success rate rises from 88\% to 94\% on
% \textsc{TurnOnElectricKettle}, from 76\% to 94\% on
% \textsc{SlideDishwasherRack}, and from 82\% to 96\% on
% \textsc{CloseToasterOvenDoor}. Because the underlying VLA is unchanged, these
% discontinuous gains reflect an improvement in the harness's ability to
% detect and repair embodied execution failures, rather than additional policy
% training.

% The three final repairs also reveal distinct physical causes. For
% \textsc{TurnOnElectricKettle}, the critic finds that, after the failed
% attempt, simply re-aligning the end-effector (EEF) with the target is enough
% to restore the geometry expected by the VLA. For
% \textsc{SlideDishwasherRack}, the key failure occurs when contact is lost
% during the push; the recovery therefore places the EEF at the middle of the
% dishwasher rack, re-establishing a centered contact configuration before the
% VLA resumes. For \textsc{CloseToasterOvenDoor}, the important correction is
% made before execution: placing the EEF underneath the door moves the initial
% state into the VLA's \emph{in-domain} region, making the subsequent closing
% motion recoverable. Thus, the Aha is not an arbitrary waypoint tweak; it is
% the identification of the physical state variable that must be restored for
% the VLA to operate reliably.

% \subsubsection{"Aha" Moments on Libero-Pro}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{figs/experiment-results/aha-case-t2-t8-s6.pdf}
%     \caption{\textbf{Representative Aha moments on LIBERO-Pro Goal.}
%     Example cases from the Reflection \& Evolve process illustrate how
%     rollout failures are converted into corrective strategies and subsequently
%     reused to recover from previously unsuccessful executions under
%     LIBERO-Pro perturbations.}
%     \label{fig:Libero-aha-case}
% \end{figure}

% Figure~\ref{fig:Libero-aha-case} shows three representative Aha moments
% during Critic--Recovery refinement. The plotted points are selected cumulative
% internal versions, rather than additional VLA training rounds or independent
% outer-loop promotions. The underlying VLA remains unchanged throughout, and
% there can be multiple unshown diagnosis and repair attempts between adjacent
% checkpoints.

% For Goal-T2, the task is to place a wine bottle inside a bowl. Pure VLA
% achieves $2/20$ success ($10\%$). The first revision introduces pregrasp
% staging, which improves the initial approach geometry but does not prevent
% object loss or premature release during transport. It therefore yields only a
% small increase to $3/20$ ($15\%$). The Aha occurs when the agent identifies
% \emph{grasp retention} as the decisive physical state. A retained-object Critic
% verifies that the bottle is securely held before invoking controlled transport
% and placement, raising success to $19/20$ ($95\%$).

% Goal-T8 similarly requires placing a wine bottle on a plate. Pregrasp recovery
% improves success from $1/20$ ($5\%$) to $2/20$ ($10\%$), but weak grasps and
% object loss during lifting remain unresolved. The second revision therefore
% monitors contact, grasp, and retention during execution. Transport begins only
% after stable retention is verified, after which the recovery completes the
% placement. This raises success to $12/20$ ($60\%$), although some
% plate-specific placement errors remain.

% For Goal-S6, the task is to place the cream cheese at the designated bowl
% target. The first revision adds a release gate that rejects gripper opening
% while the object is retained but the target relation remains unsatisfied.
% Because this gate acts only after a successful approach and grasp, it improves
% success only from $0/20$ to $1/20$ ($5\%$). The second revision moves the
% Critic before contact: sustained motion without progress toward the designated
% cream-cheese object triggers a calibrated semantic pick-and-place recovery.
% By repairing approach, grasp, transport, and placement together, success rises
% sharply to $18/20$ ($90\%$).

% Across all three tasks, the early revision repairs a visible local symptom and
% can rescue only episodes that reach the corresponding stage. The Aha revision
% instead identifies and restores the physical state required by the VLA:
% stable retained grasp for Goal-T2 and Goal-T8, and correct semantic approach
% for Goal-S6. Thus, the discontinuous gains arise from improved embodied failure
% detection and recovery, rather than additional policy training or arbitrary
% waypoint tuning.


\subsection{Physical Intelligence ``Aha'' Moments}

To validate that Z-Harness enables discontinuous capability gains through physical intelligence rather than additional policy training, we analyze the fine-grained evolutionary trajectory within individual outer-loop cycles. We present \textbf{``Aha'' moments}—instances where the system transitions from stagnant performance to high success rates by identifying and resolving the true physical bottleneck of a task.

We define an ``Aha'' moment empirically by tracking success rates across \textbf{selected cumulative internal versions} within the evolution of a single failure cluster. These checkpoints (v0, v1, v2) represent intermediate refinements made by the Evolutionary Agent during offline diagnosis and repair, rather than separate outer-loop rollouts or additional VLA training. The base VLA policy remains frozen throughout.

Through case studies on representative tasks from RoboCasa and LIBERO-Pro, we demonstrate that:
\begin{enumerate}
\item \textbf{Stagnant Early Repairs:} Early revisions often yield marginal gains because they address local symptoms or overfit specific failure episodes, leading to performance plateaus.
\item \textbf{Bottleneck Identification:} A true ``Aha'' moment occurs when the agent isolates the critical physical state variable (e.g., grasp retention, end-effector re-alignment, or semantic approach geometry) required to restore the VLA's execution to its in-domain region.
\item \textbf{Discontinuous Scaling:} Resolving this root bottleneck produces a sharp, discontinuous increase in success rate, demonstrating that the harness acquires reusable embodied intelligence rather than task-specific trajectory tweaks.
\end{enumerate}


\subsubsection{``Aha'' Moments on LIBERO-Pro}
\begin{figure}[h]
\centering
\vspace{-5mm}
\includegraphics[width=0.95\linewidth]{figs/experiment-results/aha-case-t2-t8-s6.pdf}
\caption{\textbf{Physical-intelligence ``Aha'' moments on LIBERO-Pro.} Similar to RoboCasa, v0 denotes the Pure-VLA baseline and v1 represents early symptomatic repairs (e.g., staging or local gates) that yield stagnant performance. The ``Aha'' at v2 occurs when the agent identifies and resolves the decisive physical bottleneck (e.g., grasp retention or semantic approach), triggering a sharp increase in execution reliability.}
\label{fig:Libero-aha-case}
\end{figure}

Figure~\ref{fig:Libero-aha-case} shows representative ``Aha'' moments on LIBERO-Pro, where internal evolution progresses from symptomatic fixes to root-cause repairs. The checkpoints v0, v1, and v2 mirror the stagnant-to-breakthrough trajectory observed in RoboCasa.

For \textbf{Goal-T2} (placing a bottle in a bowl), the v1 revision introduces pre-grasp staging to improve approach geometry. However, performance remains stagnant ($10\% \rightarrow 15\%$) because it fails to address object loss during transport. The ``Aha'' occurs at v2, when the agent identifies \emph{grasp retention} as the decisive bottleneck. Implementing a retained-object critic that verifies stability before transport triggers a discontinuous jump to 95\% success.

A similar plateau appears in \textbf{Goal-T8}. The v1 revision improves success only marginally ($5\% \rightarrow 10\%$) as weak grasps during lifting remain unresolved. The v2 ``Aha'' moment involves implementing a recovery that monitors the full contact--grasp--retention sequence, ensuring stable retention before initiating transport. This raises success sharply to 60\%, as the system finally masters the physical transition from acquisition to transport.

In \textbf{Goal-S6} (placing cream cheese), the early v1 revision focuses on a release gate to prevent premature dropping. Because this only repairs a late-stage symptom, success stays stagnant at 5\%. The v2 ``Aha'' moment shifts the focus to the \emph{pre-contact phase}: the agent recognizes that the primary bottleneck is a lack of semantic progress during approach. By implementing a calibrated semantic pick-and-place recovery, the system resolves approach, grasp, and transport failures simultaneously, resulting in a sharp rise to 90\% success.

Across both benchmarks, these ``Aha'' moments confirm that the scalable unit of physical intelligence is the identification of state variables—such as grasp stability or approach geometry—that must be restored for reliable VLA execution.


\subsubsection{``Aha'' Moments on RoboCasa}
\begin{figure*}[h]
\centering
\vspace{-5mm}
\includegraphics[width=0.95\textwidth]{figs/robocasa-results/fig_use/loop2_aha_moments.pdf}
\vspace{-5mm}
\caption{\textbf{Physical-intelligence ``Aha'' moments on RoboCasa.} L2-v0 is the original Pure-VLA baseline, while L2-v1 is an intermediate internal version. The flat L2-v0--L2-v1 segments summarize a period where early candidate fixes overfit individual failures. Once the agent identifies the key physical bottleneck (e.g., EEF alignment or centered contact), L2-v2 produces a sharp success-rate increase.}
\label{fig:robocasa-loop2-aha}
\end{figure*}

Figure~\ref{fig:robocasa-loop2-aha} illustrates this phenomenon on three representative RoboCasa tasks. We report success rates at three selected checkpoints within Loop-2 Stage-2. L2-v0 is the Pure-VLA baseline. L2-v1 represents an intermediate state where the agent is still analyzing failures and repeatedly revising the critic and recovery implementations. During this phase, most revisions produce only marginal gains or overfit observed failures, leaving success rates near the baseline.

An ``Aha'' moment occurs at L2-v2, where the internal version finally isolates the actual physical bottleneck. Success rates rise sharply: from 88\% to 94\% on \textsc{TurnOnElectricKettle}, 76\% to 94\% on \textsc{SlideDishwasherRack}, and 82\% to 96\% on \textsc{CloseToasterOvenDoor}. For \textsc{TurnOnElectricKettle}, the ``Aha'' was recognizing that simple EEF re-alignment restores the geometry expected by the VLA. For \textsc{SlideDishwasherRack}, the key was re-establishing centered contact after contact loss. These discontinuous gains reflect the harness's improved ability to restore the required physical state for the frozen VLA.







\subsection{Physical Intelligence Scaling and Zero-shot Capability}

We investigate the scaling of physical intelligence along two complementary axes: (1) \textbf{Intra-task scaling}, which measures how performance improves as a task accumulates Critic--Recovery mechanisms through reflection-driven evolution; and (2) \textbf{Cross-task zero-shot transfer}, which examines whether mechanisms discovered on a source task can be applied to unevolved target tasks sharing similar physical failure modes. Throughout all experiments, the underlying VLA policy remains frozen.





\subsubsection{Scaling and Zero-shot Capability on LIBERO-Pro}

\paragraph{Scaling through cumulative evolution.}
\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/experiment-results/Libero-goal-t-aha-average-standardized.pdf}
        \caption{Task/instruction-redirection (T).}
        \label{fig:goal-t-average}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/experiment-results/Libero-goal-s-aha-average-standardized.pdf}
        \caption{Swap/position-swap (S).}
        \label{fig:goal-s-average}
    \end{subfigure}
    \caption{\textbf{Cumulative physical-intelligence scaling on LIBERO-Pro
    Goal.} Average performance across ten tasks under Goal-T and Goal-S
    perturbations. Each point denotes a selected cumulative harness version.
    The base VLA is frozen throughout evolution.}
    \label{fig:Libero-aha-average}
\end{figure}



\begin{figure}[!h]
    \centering
    \includegraphics[width=0.75\linewidth]{figs/experiment-results/Scaling/Libero-T-scaling-font-2.5x-cropped.pdf}
    \caption{\textbf{Cross-task scaling from the Goal-T8 source task.}
    Three cumulative Critic--Recovery capabilities discovered on Goal-T8 are
    transferred to Goal-T2, Goal-T6, and Goal-S3. Curves report complete
    fixed-seed evaluations of each cumulative stack. Shaded regions denote
    Wilson $95\%$ confidence intervals. The right-hand frames illustrate the
    corresponding failure and recovery mechanisms rather than additional
    transfer measurements.}
    \label{fig:libero-t-transfer-scaling}
\end{figure}
Figure~\ref{fig:Libero-aha-average} reports the performance scaling on LIBERO-Pro Goal-T and Goal-S. As the harness accumulates Critic--Recovery mechanisms, the average success rate increases from $31.0\%$ to $92.5\%$ on Goal-T and from $38.0\%$ to $89.0\%$ on Goal-S. This improvement is achieved without increasing model capacity or fine-tuning weights. Instead, successive reflection rounds identify and repair recurring \textit{physical bottlenecks}, such as incorrect approach geometry, unstable grasp retention, and incomplete task relations. These results suggest that physical execution reliability can scale through the cumulative acquisition of compact runtime mechanisms.




\paragraph{Zero-shot Capability on Goal-T.}
We evaluate whether mechanisms discovered during evolution encode reusable physical principles. Figure~\ref{fig:libero-t-transfer-scaling} uses Goal-T8 (placing a wine bottle) as the source task. Three cumulative capabilities were discovered: (1) pre-grasp staging, (2) a grasp-retention Critic, and (3) a failure-gated retry. When applied \textit{zero-shot} to Goal-T2, Goal-T6, and Goal-S3, these mechanisms yield significant performance gains (e.g., $9/20 \rightarrow 20/20$ on Goal-S3). The transfer succeeds because the mechanisms operate on \textit{task-independent physical variables}---such as EEF alignment and contact stability---rather than memorizing source-task trajectories.


% \begin{wrapfigure}{r}{0.7\textwidth}
%     \vspace{-10pt}
%     \centering
%     \includegraphics[width=\linewidth]{figs/experiment-results/Scaling/Libero-S-scaling-evidence-final-font-2.5x-cropped.pdf}
%     \caption{\textbf{Cross-task scaling from the Goal-S5 source task.}
%     Cumulative Critic--Recovery capabilities discovered on Goal-S5 are
%     transferred to Goal-S3, Goal-S4, and Goal-S9. Within each task, all four
%     arms use the same fixed seeds, policy RNGs, checkpoint, and execution
%     budget. Shaded regions denote Wilson $95\%$ confidence intervals.}
%     \label{fig:libero-s-transfer-scaling}
%     \vspace{-10pt}
% \end{wrapfigure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{figs/experiment-results/Scaling/Libero-S-scaling-evidence-final-font-2.5x-cropped.pdf}
    \caption{\textbf{Cross-task scaling from the Goal-S5 source task.}
    Cumulative Critic--Recovery capabilities discovered on Goal-S5 are
    transferred to Goal-S3, Goal-S4, and Goal-S9. Within each task, all four
    arms use the same fixed seeds, policy RNGs, checkpoint, and execution
    budget. Shaded regions denote Wilson $95\%$ confidence intervals.}
    \label{fig:libero-s-transfer-scaling}
    \vspace{-5mm}
\end{figure}
\paragraph{Zero-shot Capability on Goal-S.}
\begin{wrapfigure}{r}{0.45\textwidth}
    \centering
    \includegraphics[width=0.45\textwidth]
    {figs/robocasa-results/fig_use/atomic_18task_general_gain.pdf}
    \caption{\textbf{Cumulative reflection scaling across 18 RoboCasa tasks.}
    The macro-average success rate increases from 73.56\% for the frozen
    parent harness to 78.71\%, 84.85\%, 90.54\%, and 93.56\% after four
    cumulative global repair rounds. Each checkpoint retains the previously
    validated critic, recovery, and tool capabilities.}
    \label{fig:robocasa-atomic-scaling}
    \vspace{-30pt}
\end{wrapfigure}
Figure~\ref{fig:libero-s-transfer-scaling} provides a complementary study using Goal-S5 as the source task. The evolved mechanisms include contact-qualified takeovers based on EEF--object proximity and a stalled-command carry gate for robust transport. Without changing the frozen policy, the same cumulative stack was evaluated \textit{zero-shot} on Goal-S3, Goal-S4, and Goal-S9. The results show that mechanisms learned from a single task can successfully repair shared grasp, contact, and transport failures across multiple unevolved tasks, demonstrating that the scalable unit is a reusable mapping from physical failure states to recovery behaviors.

\subsubsection{Scaling and Zero-shot Capability on RoboCasa}




\paragraph{Scaling through cumulative evolution.}
The aggregate scaling trend on 18 RoboCasa tasks is shown in Figure~\ref{fig:robocasa-atomic-scaling}. Through four rounds of global reflection and repair, the macro-average success rate increases from $73.56\%$ to $93.56\%$. Since the VLA is frozen, this $20.00$ percentage-point gain reflects the accumulation of validated execution knowledge within the harness. The scaling variable here is the cumulative reflection experience, which continuously improves the capability of a fixed policy by addressing deeper physical bottlenecks.

\paragraph{Zero-shot transfer of Pick-and-Place capabilities.}


We examine the zero-shot transferability of mechanisms discovered on \textsc{PnP-Stove} (Figure~\ref{fig:robocasa-pnp-scaling}). Three cumulative rounds on the source task produced: (1) \textit{pre-grasp alignment}, (2) \textit{re-grasp after grasp loss}, and (3) \textit{stable placement}. Without any additional training or evolution loops, we apply this cumulative stack to \textsc{PnP-Sink}, \textsc{PnP-Cabinet}, and \textsc{PnP-Toaster}. The macro-average success rate over these transfer tasks increases from $64\%$ to $84\%$. This $20$ percentage-point zero-shot gain demonstrates that the agent learns general pick-and-place principles that transcend specific object identities or furniture geometries.
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.95\textwidth]
    {figs/robocasa-results/fig_use/scaling_robocasa.pdf}
    \caption{\textbf{Reflection-driven scaling and transfer on PnP tasks.}
    On PnP-Stove, successive rounds add object-relative pregrasp alignment,
    bounded regrasp after grasp loss, and stable placement. The lower panels
    apply the cumulative checkpoints to PnP-Sink, PnP-Cabinet, and PnP-Toaster
    without an additional training or evolution loop. The right-hand panels
    show the failure signatures identified by the critic and the corresponding
    recoveries.}
    \label{fig:robocasa-pnp-scaling}
\end{figure*}


\paragraph{Zero-shot transfer of Articulated interaction capabilities.}

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.95\textwidth]
    {figs/robocasa-results/fig_use/scaling_robocasa_2.pdf}
    \caption{\textbf{Reflection-driven scaling and transfer on articulated
    interaction tasks.} On TurnOffStove, successive rounds add target
    localization, collision-aware pre-contact approach, and stable
    EEF--target contact. The lower panels apply the cumulative checkpoints to
    TurnOnSinkFaucet, OpenCabinet, and TurnOnMicrowave without an additional
    training or evolution loop. The right-hand panels show the diagnosed
    target, approach, and contact failures together with the recovered states.}
    \label{fig:robocasa-turnoff-scaling}
\end{figure*}

A second study focuses on \textsc{TurnOffStove}, where the agent evolves (1) \textit{target localization}, (2) \textit{collision-aware approach}, and (3) \textit{stable-contact} skills (Figure~\ref{fig:robocasa-turnoff-scaling}). These skills describe physical invariants shared by many articulated-interaction tasks. We evaluate these source-task mechanisms \textit{zero-shot} on \textsc{TurnOnSinkFaucet}, \textsc{OpenCabinet}, and \textsc{TurnOnMicrowave}. The transfer-task macro-average increases from $64\%$ to $80\%$, a $16$ percentage-point improvement without target-task adaptation. These results confirm that the scalable unit in our framework is not a task-specific trajectory, but a reusable mapping from observable physical failure states to robust recovery behaviors.





% \subsection{Physical Intelligence Scaling and Zero-shot Capability} 

% \subsubsection{Scaling and Zero-shot Capability on Libero-Pro}

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}[t]{0.48\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/experiment-results/Libero-goal-t-aha-average-standardized.pdf}
%         \caption{Task/instruction-redirection (T).}
%         \label{fig:goal-t-average}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.48\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/experiment-results/Libero-goal-s-aha-average-standardized.pdf}
%         \caption{Swap/position-swap (S).}
%         \label{fig:goal-s-average}
%     \end{subfigure}
%     \caption{\textbf{Cumulative physical-intelligence scaling on LIBERO-Pro
%     Goal.} Average performance across ten tasks under Goal-T and Goal-S
%     perturbations. Each point denotes a selected cumulative harness version.
%     The base VLA is frozen throughout evolution.}
%     \label{fig:Libero-aha-average}
% \end{figure}
% We study physical-intelligence scaling on LIBERO-Pro along two complementary
% axes. First, we measure how performance improves as each task accumulates
% Critic--Recovery mechanisms during evolution. Second, we examine whether
% mechanisms discovered on one source task can be transferred to tasks with
% similar physical failure modes. In all cases, the base VLA remains frozen.
% Each plotted checkpoint evaluates a complete cumulative harness version,
% rather than an action prefix within one episode.

% \paragraph{Scaling through cumulative evolution.}
% Figure~\ref{fig:Libero-aha-average} reports the average success rate over the
% ten Goal-T and ten Goal-S tasks as additional Critic--Recovery mechanisms are
% incorporated. The average success rate increases from $31.0\%$ to $92.5\%$ on
% Goal-T and from $38.0\%$ to $89.0\%$ on Goal-S. The improvement is not obtained
% by increasing model capacity or fine-tuning the VLA. Instead, successive
% versions identify and repair recurring physical bottlenecks, including
% incorrect approach geometry, unstable grasp retention, premature release,
% stalled execution, and incomplete task relations. The resulting trend shows
% that physical execution reliability can scale through the cumulative
% acquisition of compact runtime mechanisms.
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figs/experiment-results/Scaling/Libero-T-scaling-font-2.5x-cropped.pdf}
%     \caption{\textbf{Cross-task scaling from the Goal-T8 source task.}
%     Three cumulative Critic--Recovery capabilities discovered on Goal-T8 are
%     transferred to Goal-T2, Goal-T6, and Goal-S3. Curves report complete
%     fixed-seed evaluations of each cumulative stack. Shaded regions denote
%     Wilson $95\%$ confidence intervals. The right-hand frames illustrate the
%     corresponding failure and recovery mechanisms rather than additional
%     transfer measurements.}
%     \label{fig:libero-t-transfer-scaling}
% \end{figure}

% \paragraph{Zero-shot Capability on Goal-T.}
% Figure~\ref{fig:libero-t-transfer-scaling} uses Goal-T8, which requires placing
% a wine bottle on a plate, as the source task. Three cumulative capabilities are
% discovered during its evolution: (1) pregrasp staging that establishes a stable
% approach configuration; (2) a retained-object Critic that verifies grasp
% retention before transport; and (3) a failure-gated slow retry with controlled
% closing, holding, lifting, and vertical-first transport. These additions raise
% Goal-T8 from $1/20$ to $2/20$, $16/20$, and finally $18/20$ successes.


% We then apply the same cumulative stack to three distinct transfer tasks.
% Goal-T2 improves from $4/20$ to $8/20$ and $18/20$ after the first two
% capabilities, while Goal-T6 improves from $4/20$ to $9/20$, $18/20$, and
% $19/20$. On Goal-S3, which changes both the manipulated object and the target
% relation, performance increases from $9/20$ to $17/20$, $19/20$, and $20/20$.
% The transfer succeeds because the mechanisms operate on task-independent
% physical variables---EEF alignment, contact, gripper state, grasp retention,
% execution progress, and relation satisfaction---rather than memorizing the
% source task's object identities or trajectory. Skill~3 produces no additional
% gain on Goal-T2 because the preceding stack already resolves its dominant
% failure mode.


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figs/experiment-results/Scaling/Libero-S-scaling-evidence-final-font-2.5x-cropped.pdf}
%     \caption{\textbf{Cross-task scaling from the Goal-S5 source task.}
%     Cumulative Critic--Recovery capabilities discovered on Goal-S5 are
%     transferred to Goal-S3, Goal-S4, and Goal-S9. Within each task, all four
%     arms use the same fixed seeds, policy RNGs, checkpoint, and execution
%     budget. Shaded regions denote Wilson $95\%$ confidence intervals.}
%     \label{fig:libero-s-transfer-scaling}
% \end{figure}
% \paragraph{Zero-shot on Goal-S.}
% Figure~\ref{fig:libero-s-transfer-scaling} provides a complementary controlled
% study using Goal-S5 as the source task. Its cumulative stack consists of:
% (1) a retained-grasp or timeout-triggered takeover; (2) a contact-qualified
% takeover based on EEF--object proximity; and (3) robust transport with a
% bounded retry and a state-qualified stalled-command carry gate. On a fixed
% five-seed block, the source-task success rate increases from $0/5$ to $2/5$,
% $4/5$, and $5/5$.

% Without changing the frozen policy or task-specific action interface, the same
% stack is evaluated on fixed seed and policy-RNG blocks for Goal-S3, Goal-S4,
% and Goal-S9. Their cumulative success rates are respectively
% $1/5 \rightarrow 4/5 \rightarrow 4/5 \rightarrow 5/5$,
% $0/5 \rightarrow 5/5 \rightarrow 5/5 \rightarrow 5/5$, and
% $2/5 \rightarrow 5/5 \rightarrow 5/5 \rightarrow 5/5$.
% These controlled development-block results show that a mechanism learned from
% one task can repair shared grasp, contact, and transport failures on other
% tasks. They are intended as transfer diagnostics rather than additional blind
% held-out evaluations.



% Together, these results reveal two forms of scaling. Within a task, performance
% increases as the harness accumulates mechanisms that address progressively
% deeper physical bottlenecks. Across tasks, the same mechanisms remain useful
% whenever the underlying failure signatures are shared. Thus, the scalable unit
% is not a task-specific trajectory, but a reusable mapping from observable
% physical failure states to bounded recovery behaviors.

% \subsubsection{Scaling and Zero-shot Capability on Robocasa}


% \begin{wrapfigure}{r}{0.48\textwidth}
%     \vspace{-10pt}
%     \centering
%     \includegraphics[width=0.46\textwidth]
%     {figs/robocasa-results/fig_use/atomic_18task_general_gain.pdf}
%     \caption{\textbf{Cumulative reflection scaling across 18 RoboCasa tasks.}
%     The macro-average success rate increases from 73.56\% for the frozen
%     parent harness to 78.71\%, 84.85\%, 90.54\%, and 93.56\% after four
%     cumulative global repair rounds. Each checkpoint retains the previously
%     validated critic, recovery, and tool capabilities.}
%     \label{fig:robocasa-atomic-scaling}
%     \vspace{-10pt}
% \end{wrapfigure}

% \paragraph{Scaling through cumulative evolution} We study scaling through cumulative, reflection-driven harness evolution. The
% underlying VLA policy, simulator, and evaluation protocol remain fixed
% throughout the process. After each rollout batch, the Evolutionary Agent
% reflects on the observed failures, identifies recurring physical bottlenecks,
% and proposes critic--recovery updates. Only candidates that pass validation are
% added to the harness, and all later checkpoints retain the capabilities
% validated in earlier rounds.

% The scaling variable is therefore the cumulative reflection and repair
% experience processed by the harness, rather than the parameter count of the
% VLA. This design allows us to ask two questions: whether additional reflection
% rounds continuously improve the source-task capability of a frozen policy, and
% whether the resulting skills encode reusable physical principles that transfer
% to related tasks. For the transfer experiments, we do not run an additional
% training or evolution loop on the target task; only the minimal object- or
% scene-level adaptation needed to instantiate the same skill is performed.




% Figure~\ref{fig:robocasa-atomic-scaling} gives the aggregate scaling result.
% Across the 18 RoboCasa Atomic-Seen tasks, the macro-average success rate
% increases from 73.56\% for the parent harness to 78.71\% after the first
% global repair round, 84.85\% after the second, 90.54\% after the third, and
% 93.56\% after the fourth. Since the base VLA and simulator are unchanged, the
% 20.00 percentage-point improvement reflects the accumulation of validated
% execution knowledge in the harness rather than policy-weight updates. The two
% case studies below explain which physical capabilities are acquired during
% this process and how they transfer within their respective task families.

% \paragraph{PnP-Stove: reusable pick-and-place capabilities.}

% We first study \textsc{PnP-Stove}, in which the robot must grasp an object,
% transport it, and place it on the stove. Figure~\ref{fig:robocasa-pnp-scaling}
% shows three successive reflection rounds, each resolving a different
% failure mode.

% In Round~1, the agent learns an object-relative
% \emph{pregrasp-alignment skill}. When the VLA approaches the object from an
% unreliable pose, the recovery first moves the EEF to a feasible pregrasp
% configuration and then executes the acquisition motion. This prevents the
% system from repeatedly issuing the same misaligned grasp.

% In Round~2, the agent learns bounded \emph{regrasp after grasp loss}. When the
% object is dropped or the grasp predicate becomes invalid, the harness releases
% and restages the gripper, selects a new feasible grasp proposal, and checks
% grasp stability before returning control to the VLA. The recovery therefore
% changes the failed contact configuration instead of replaying the failed
% trajectory.

% In Round~3, the agent learns \emph{stable placement}. Near the destination,
% the recovery verifies object support and placement stability before release,
% then retreats until the EEF is safely separated. This prevents unstable
% release and premature termination near the final placement.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.98\textwidth]
%     {figs/robocasa-results/fig_use/scaling_robocasa.pdf}
%     \caption{\textbf{Reflection-driven scaling and transfer on PnP tasks.}
%     On PnP-Stove, successive rounds add object-relative pregrasp alignment,
%     bounded regrasp after grasp loss, and stable placement. The lower panels
%     apply the cumulative checkpoints to PnP-Sink, PnP-Cabinet, and PnP-Toaster
%     without an additional training or evolution loop. The right-hand panels
%     show the failure signatures identified by the critic and the corresponding
%     recoveries.}
%     \label{fig:robocasa-pnp-scaling}
% \end{figure*}

% The source-task success rate increases from 78\% for Pure VLA to 84\%, 94\%,
% and 96\% after the three cumulative rounds. These improvements are not tied to
% the appearance of the stove or to one successful object trajectory. Pregrasp
% alignment, grasp retention, and stable placement are recurring requirements of
% pick-and-place interaction.

% The same checkpoints consequently transfer to related PnP tasks without
% another training or evolution procedure. Success increases from 58\% to 82\%
% on PnP-Sink, from 62\% to 80\% on PnP-Cabinet, and from 72\% to 90\% on
% PnP-Toaster. The macro-average over the three transfer tasks increases from
% 64\% to 84\%, an absolute gain of 20 percentage points. This result suggests
% that the agent learns reusable pick-and-place capabilities rather than
% memorizing a task-specific trajectory.


% \paragraph{TurnOffStove: reusable target, approach, and contact capabilities.}

% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=0.9\textwidth]
%     {figs/robocasa-results/fig_use/scaling_robocasa_2.pdf}
%     \caption{\textbf{Reflection-driven scaling and transfer on articulated
%     interaction tasks.} On TurnOffStove, successive rounds add target
%     localization, collision-aware pre-contact approach, and stable
%     EEF--target contact. The lower panels apply the cumulative checkpoints to
%     TurnOnSinkFaucet, OpenCabinet, and TurnOnMicrowave without an additional
%     training or evolution loop. The right-hand panels show the diagnosed
%     target, approach, and contact failures together with the recovered states.}
%     \label{fig:robocasa-turnoff-scaling}
% \end{figure*}

% We next study \textsc{TurnOffStove}, where the robot must identify the correct
% knob, approach it without collision, and execute the turning motion only after
% establishing stable EEF--target contact. Figure~\ref{fig:robocasa-turnoff-scaling}
% shows how the agent acquires these capabilities over three reflection rounds.

% In Round~1, the agent learns a \emph{target-localization skill}. Failure
% analysis shows that the VLA can act on a nearby but incorrect knob even when
% the subsequent motion is otherwise valid. The evolved critic therefore checks
% the target identity and position, while the recovery redirects the EEF toward
% the correct target.

% In Round~2, the agent learns a collision-aware
% \emph{pre-contact approach skill}. Instead of moving directly toward the
% target from an arbitrary configuration, the recovery constructs a feasible
% relative EEF pose, avoids nearby obstacles, and aligns the end-effector before
% initiating contact. This addresses both misaligned approaches and collisions
% during the approach phase.

% In Round~3, the agent learns a \emph{stable-contact skill}. Before executing
% the turning action, the critic verifies that the EEF and target have formed a
% sufficiently stable contact. If the contact is misaligned or unstable, the
% harness corrects the contact configuration before allowing the VLA action to
% continue.



% These additions increase TurnOffStove success from 74\% for Pure VLA to
% 82\%, 84\%, and 92\% after the three cumulative rounds. The acquired skills
% again describe physical invariants shared by related articulated-interaction
% tasks rather than a single knob configuration.

% Without target-task training or another evolution loop, the cumulative
% checkpoints improve TurnOnSinkFaucet from 74\% to 90\%, OpenCabinet from 62\%
% to 78\%, and TurnOnMicrowave from 56\% to 72\%. The transfer-task
% macro-average increases from 64\% to 80\%, an absolute gain of 16 percentage
% points. The OpenCabinet curve plateaus after Round~2, showing that scaling is
% mechanism-dependent: a newly acquired skill helps tasks that share its
% physical bottleneck, but does not resolve unrelated failure modes.

% Together, the aggregate curve and the two case studies show that reflection
% provides more than repeated attempts on individual episodes. As the number of
% reflection and repair rounds increases, the harness accumulates executable
% skills for pregrasp alignment, regrasp, stable placement, target localization,
% approach geometry, and contact stability. These skills improve the original
% task and transfer to related RoboCasa tasks, demonstrating
% reflection-driven capability scaling for a frozen VLA policy.






\subsection{Results on Simulation benchmark}
\paragraph{RoboCasa}
Table~\ref{tab:robocasa-atomic} reports the success rate on all 18
RoboCasa Atomic-Seen tasks. We use compact task identifiers in the main text;
their official RoboCasa names are listed in
Appendix~\ref{app:atomic-task-mapping}. Compared with the frozen GR00T
post-trained VLA, \sys improves the macro-average success rate from 73.56\%
to 93.56\%, an absolute gain of 20.00 percentage points. The improvement is
consistent across all tasks and is especially large on contact-rich or
long-horizon manipulation tasks such as T4, T5, and T15.
\begin{table}[h]
    \centering
    \caption{\textbf{Success rates (\%) on 18 RoboCasa Atomic-Seen tasks.}
    Task identifiers follow Appendix~\ref{app:atomic-task-mapping}. The best
    result for each task is shown in bold. ``Avg.'' is the macro-average over
    all 18 tasks.}
    \label{tab:robocasa-atomic}
    \small
    \setlength{\tabcolsep}{3.2pt}
    \renewcommand{\arraystretch}{1.08}
    \resizebox{0.7\columnwidth}{!}{%
    \begin{tabular}{lcccccccccc}
        \toprule
        \textbf{Method} & \textbf{T1} & \textbf{T2} & \textbf{T3}
        & \textbf{T4} & \textbf{T5} & \textbf{T6} & \textbf{T7}
        & \textbf{T8} & \textbf{T9} & \textbf{Avg.} \\
        \midrule
        Pure VLA (GR00T)
        & 78 & 74 & 78 & 58 & 48 & 62 & 72 & 74 & 70 & 73.56 \\
        \sys
        & \textbf{96} & \textbf{92} & \textbf{94} & \textbf{96}
        & \textbf{86} & \textbf{80} & \textbf{96} & \textbf{96}
        & \textbf{86} & \textbf{93.56} \\
        \midrule
        \textbf{Method} & \textbf{T10} & \textbf{T11} & \textbf{T12}
        & \textbf{T13} & \textbf{T14} & \textbf{T15} & \textbf{T16}
        & \textbf{T17} & \textbf{T18} & \textbf{Avg.} \\
        \midrule
        Pure VLA (GR00T)
        & 62 & 92 & 76 & 88 & 96 & 50 & 90 & 82 & 74 & 73.56 \\
        \sys
        & \textbf{94} & \textbf{98} & \textbf{94} & \textbf{94}
        & \textbf{100} & \textbf{100} & \textbf{94} & \textbf{96}
        & \textbf{92} & \textbf{93.56} \\
        \bottomrule
    \end{tabular}%
    }
\end{table}



\paragraph{Libero-Pro}
Table~\ref{tab:libero-pro} reports results on 40 task-setting pairs across
the Goal and LIBERO-10 suites. Compared with the frozen $\pi_{0.5}$ baseline,
\sys improves the overall macro-average from 32.00\% to 71.13\%, an absolute
gain of 39.13 percentage points. The gains are largest on Goal (T) and Goal
(S), whose averages increase from 31.0\% to 92.5\% and from 38.0\% to 89.0\%,
respectively. On LIBERO-10, \sys improves the T and S settings from 50.0\% to
63.0\% and from 9.0\% to 40.0\%. Overall, \sys improves 32 task-setting pairs
and matches the baseline on the remaining eight.

\begin{table}[h]
\centering
\caption{\textbf{Success rates (\%) on LIBERO-Pro.} The best result for each
task is shown in bold. ``Average'' is the macro-average over 10 tasks.}
\label{tab:libero-pro}
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.08}
\resizebox{\linewidth}{!}{
\begin{tabular}{llccccccccccc}
\toprule
\textbf{Setting} & \textbf{Method}
& \textbf{Task 0} & \textbf{Task 1} & \textbf{Task 2} & \textbf{Task 3}
& \textbf{Task 4} & \textbf{Task 5} & \textbf{Task 6} & \textbf{Task 7}
& \textbf{Task 8} & \textbf{Task 9} & \textbf{Average} \\
\midrule

\multirow{2}{*}{\textbf{Goal (T)}}
& $\pi_{0.5}$
& 0.0 & 95.0 & 10.0 & 0.0 & \textbf{100.0} & 0.0 & 20.0 & 80.0 & 5.0 & 0.0 & 31.0 \\
& \sys
& \textbf{80.0} & \textbf{100.0} & \textbf{95.0} & \textbf{80.0}
& \textbf{100.0} & \textbf{100.0} & \textbf{95.0} & \textbf{95.0}
& \textbf{80.0} & \textbf{100.0} & \textbf{92.5} \\
\midrule

\multirow{2}{*}{\textbf{Goal (S)}}
& $\pi_{0.5}$
& 0.0 & 60.0 & 0.0 & 45.0 & 0.0 & 0.0 & 0.0
& \textbf{100.0} & \textbf{100.0} & 75.0 & 38.0 \\
& \sys
& \textbf{90.0} & \textbf{65.0} & \textbf{80.0} & \textbf{85.0}
& \textbf{95.0} & \textbf{95.0} & \textbf{100.0}
& \textbf{100.0} & \textbf{100.0} & \textbf{80.0} & \textbf{89.0} \\
\midrule

\multirow{2}{*}{\textbf{LIBERO-10 (T)}}
& $\pi_{0.5}$
& 5.0 & \textbf{95.0} & 95.0 & \textbf{0.0} & 0.0
& 80.0 & 85.0 & 75.0 & 65.0 & \textbf{0.0} & 50.0 \\
& \sys
& \textbf{35.0} & \textbf{95.0} & \textbf{100.0} & \textbf{0.0}
& \textbf{25.0} & \textbf{100.0} & \textbf{95.0} & \textbf{80.0}
& \textbf{100.0} & \textbf{0.0} & \textbf{63.0} \\
\midrule

\multirow{2}{*}{\textbf{LIBERO-10 (S)}}
& $\pi_{0.5}$
& 0.0 & 35.0 & 0.0 & 0.0 & 5.0 & 50.0 & 0.0
& \textbf{0.0} & \textbf{0.0} & 0.0 & 9.0 \\
& \sys
& \textbf{90.0} & \textbf{50.0} & \textbf{95.0} & \textbf{75.0}
& \textbf{15.0} & \textbf{65.0} & \textbf{5.0}
& \textbf{0.0} & \textbf{0.0} & \textbf{5.0} & \textbf{40.0} \\

\bottomrule
\end{tabular}
}
\end{table}

\paragraph{Final best accuracy vs other SOTA.}
% Libero and RoboCasa results on Atomic and Composite tasks vs. VLA models?

On LIBERO-Pro, the final \sys configuration achieves 92.5\% and 89.0\%
average success on Goal (T) and Goal (S), and 63.0\% and 40.0\% on the
corresponding LIBERO-10 settings. Compared with the strong frozen
$\pi_{0.5}$ VLA, this raises the overall average from 32.00\% to 71.13\%.
Notably, these gains require no additional VLA training: \sys improves or
matches the baseline on every task-setting pair by detecting execution
failures and applying targeted recovery at test time.



\subsection{Case Studies}
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{figs/robocasa-results/fig_use/case_study_robo.pdf}
    \caption{\textbf{A sequence of critic--recovery interventions during aPnP episode.} The VLA first picks and transports the object.  A critic detects a lost grasp and triggers a re-approach recovery; an invalid
    re-grasp pose then triggers \textsc{GraspGen} to synthesize a feasible
    grasp pose; near the goal, a final critic invokes stable \textsc{CAP}
    placement.  After each local repair, control returns to the nominal VLA
    only after the recovery state is verified.}
    \label{fig:pnp-transport-case}
\end{figure*}
\paragraph{Repeated critic--recovery interventions in Robocasa}
Figure~\ref{fig:pnp-transport-case} illustrates a representative PnP
execution in which the harness resolves several distinct failures within a
single episode.  The base VLA first completes the pick and begins transporting
the object.  When the object slips from the gripper, the runtime critic detects
the loss of grasp and interrupts the nominal trajectory.  The corresponding
recovery executes a controlled re-approach to the object and establishes a new
grasp, after which control returns to the VLA for transport.

The second intervention is triggered when the initial re-grasp pose is
infeasible.  Rather than repeatedly issuing the same motion, the critic reports
the invalid approach geometry and the recovery invokes \textsc{GraspGen} to
generate a feasible end-effector pose.  The generated pose is then executed to
re-grasp the object, restoring the contact configuration required for stable
transport.  Finally, as the object approaches the destination, the critic
detects near-goal placement risk and hands control to a stable placement
recovery based on \textsc{CAP}.  This recovery completes the final placement
before the harness verifies the re-entry conditions and terminates the episode.

This example demonstrates that the harness is not limited to a single
episode-level retry: critics can monitor the execution continuously, trigger
different recoveries for different physical failure modes, and return control
to the VLA after each local repair.  The resulting behavior is a sequence of
targeted interventions---re-approach, GraspGen-based re-grasp, and CAP-based
placement---that preserves the nominal policy while making the long-horizon
execution robust to contact and grasp failures.




\paragraph{Moving the failure frontier across promotion rounds in Libero-Pro}
Figure~\ref{fig:libero-goal-s5-case} presents the corresponding iterative
behavior in LIBERO-Pro Goal-S5, where the robot must push the plate to the
front of the stove. Unlike the RoboCasa example, the panels do not depict
multiple independent critic activations within one episode. Instead, they
summarize representative episodes from successive promotion rounds and show
how each promoted critic--recovery skill moves the earliest unresolved failure
to a later execution stage.

In Round~0, the parent VLA continues executing without a timely handoff to a
bounded recovery and eventually exhausts the episode budget. Round~1
introduces a retention-gated handoff. This resolves the absence of intervention,
but the episode now stops because a stable grasp cannot be verified. Round~2
adds a closing-contact critic and a contact-gated grasp recovery. The plate is
successfully acquired, exposing a new failure during transport: the retained
grasp is lost while carrying the plate. Thus, the failure frontier has moved
from recovery invocation, through grasp verification, to carry retention.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/experiment-results/Libero-pro-Goal-S5-case-study.pdf}
    \caption{\textbf{Critic--recovery promotion progressively moves the
    failure frontier in LIBERO-Pro Goal-S5.} The parent VLA exhausts its
    execution budget without a timely recovery handoff. Successive promotion
    rounds introduce a retention-gated handoff, a contact-gated grasp
    recovery, and a bounded re-grasp retry. Each addition resolves the
    previously exposed failure and reveals a later-stage bottleneck, until
    retained transport resumes and the official stove-front relation is
    satisfied.}
    \label{fig:libero-goal-s5-case}
\end{figure}
Round~3 addresses this later-stage failure with a bounded re-grasp retry. When
the critic detects loss of the plate during carry, the recovery does not restart
the entire episode or repeat the nominal action indefinitely. It performs a
bounded re-grasp attempt, verifies the restored retention state, and resumes
transport toward the stove-front region. The episode terminates only after the
official LIBERO relation becomes true. Importantly, Rounds~2 and~3 use the same
environment seed and policy RNG, directly isolating the contribution of the
carry-retry mechanism. Separate same-seed adjacent-round comparisons similarly
validate the retention-handoff and contact-gated grasp additions.

Together, the two case studies expose complementary forms of compositionality.
RoboCasa composes several specialized recoveries online within a single
long-horizon episode, whereas LIBERO-Pro composes promoted critic--recovery
skills across outer-loop iterations. In both cases, improvement arises from
localizing the earliest unresolved failure, applying a bounded repair, and
verifying the repaired state before allowing execution to advance.





\subsection{Z-Infra Performance Evaluation}

Z-Infra enables effective throughput scaling under high concurrency with controlled latency growth, achieving 7.7$\times$ higher throughput than \textbf{Ours without Z-Infra} and 12.8$\times$ higher than \textbf{RPent}~\cite{zhang2026harnessvla} under moderate concurrency, while reducing per-episode latency by 11.9$\times$ compared to RPent.
We evaluate throughput scaling behavior across different concurrency levels (1, 8, 16, 32, 64) on LIBERO Goal~\cite{liu2023libero}.
All experiments run on 8$\times$A100 GPUs with identical model checkpoints and action budgets.

\begin{figure}
    \centering
    \includegraphics[width=0.65\linewidth]{figs/rollout-latency.pdf}
    \caption{Per-episode latency versus concurrency. Z-Infra maintains controlled growth while baselines exhibit explosive degradation or inherently high overhead. Both baselines encounter OOM beyond concurrency 16.}
    \label{fig:rollout-latency}
\end{figure}

\paragraph{Latency Under Load.} Z-Infra maintains controlled latency growth under high concurrency, while baselines either exhibit explosive degradation or inherently high overhead. 
As shown in Figure~\ref{fig:rollout-latency}, Z-Infra's per-episode latency increases from 39s at concurrency 8 to 57s at concurrency 32 (46\% increase), then to 95s at concurrency 64. 
In contrast, Ours w/o Z-Infra experiences explosive latency degradation—from 34s at concurrency 8 to 112s at concurrency 16 (3.3$\times$ increase). 
RPent exhibits inherently high latency (392s$\to$513s), as agent-in-the-loop design requires LLM API calls at every decision point. 
Our approach reduces agent overhead by invoking agents only during offline Reflection \& Evolve phases, while online rollouts execute pure VLA policy under lightweight runtime critics. 
Z-Infra further ensures that latency growth remains sublinear even as concurrency scales, maintaining efficient resource utilization without cascading delays.
% (Figure~\ref{fig:embodiHarness_overview})
\paragraph{Throughput Scaling.} Z-Infra achieves effective throughput scaling up to hardware saturation, while baselines fail to scale beyond low concurrency levels due to resource contention. 
As shown in Figure~\ref{fig:rollout-throughput}, Z-Infra's throughput increases from 12.18 ep/min at concurrency 8 to 32.8 ep/min at concurrency 32 (2.7$\times$ speedup), reaching 22.09 ep/min at concurrency 16—7.7$\times$ higher than Ours w/o Z-Infra (2.88 ep/min) and 12.8$\times$ higher than RPent (1.72 ep/min). 
Beyond concurrency 32, throughput plateaus at 35.1 ep/min (concurrency 64), indicating saturation of the 8-GPU configuration. 
The performance gap stems from Z-Infra's persistent worker design with dynamic batching and asynchronous scheduling, which eliminates per-episode initialization overhead and maintains high GPU utilization under variable request patterns.


\begin{figure}
    \centering
    \includegraphics[width=0.65\linewidth]{figs/rollout-throughput.pdf}
    \caption{Rollout throughput versus concurrency. Z-Infra scales to 35.1 ep/min at concurrency 64, achieving 7.7× and 12.8× higher throughput than baselines at concurrency 16. Baselines fail beyond concurrency 16 due to OOM.}
    \label{fig:rollout-throughput}
\end{figure}


==> arxiv_submission/tex/introduction.tex <==
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{figs/Z_Harness_teaser.pdf}
%   \caption{\textbf{\sys closes the loop for embodied self-evolution.\ting{waiting to fill in the data blocks in the teaser figure @mingzhe @zhangchao}} Frequent runtime critics trigger recoveries during execution, while verified failures are distilled into reusable critic and recovery skills across rollouts. A hardware-decoupled rollout layer scales this process across heterogeneous environments, models, CPUs, and GPUs, enabling sustained same-task improvement, cross-task transfer, and efficient agent execution.}
%   \label{fig:teaser}
% \end{figure} 

\section{Introduction}

Physical intelligence is advancing along two complementary paths for effective scaling. The first scales end-to-end policy models, including vision-language-action models (VLAs) and world-action models (WAMs)~\cite{brohan2022rt1,brohan2023rt2,kim2024openvla,black2024pi0,black2025pi05,bjorck2025groot,li2024cogact,bu2025univla,pertsch2025fast,dreamzero2026,cosmospolicy2026,fastwam2026,yu2026wall,team2026xiaomi,lingbot_va,lingbot_vla,qwen_vla,qwen_robotmanip,kim2026rldx,jiang2025galaxea,zheng2025xvla,nvidia2026cosmos3}, trained on large-scale demonstration corpora such as DROID and Open X-Embodiment~\cite{khazatsky2024droid,oneill2023openx}.
However, embodied data remain scarce, and models trained on limited data distributions are brittle under the changing dynamics of real-world deployment~\cite{belkhale2023dataquality,ross2011reduction,nagabandi2018metarl,mandlekar2021whatmatters,simchowitz2025pitfalls,xie2023decomposinggap}; the gap from demonstration to reliable real-world execution therefore remains open.

The second path uses large language models as embodied agents to orchestrate policy models, code, tools, and control primitives~\cite{capx2026,aspire2026,xiao2026enpire,anthropic2026clauderobotics,zhang2026harnessvla}, with the aim of learning from self-exploration in environments. Though these systems alleviate limitations of end-to-end policies, existing embodied agent harnesses do not actually realize this learning. Existing embodied agent harnesses therefore remain largely open-loop: once execution begins, the agent does not continuously condition its decisions on the evolving robot-environment state, but instead follows fixed skills or preplanned trajectories and reflects only after the episode is completed. \emph{This work enables a closed-loop embodied agent harness, learning from self-exploration and demonstrating self-evolution: as rollout experience increases, the success rate continues to improve.}

Realizing closed-loop execution for embodied agents is fundamentally bottlenecked by the high-frequency interaction between robots and changing environments. Physical tasks require decisions to be coupled to the current robot and environment state, often changing within a millisecond-level latency budget~\cite{li2025holdmybeer,lee2022realtimempc}. Large agentic models cannot make decisions at this frequency in real-world systems~\cite{zhang2024hirt,yan2026actingwhileunderstanding,tan2024fouriercontroller}. Existing methods therefore perform reflection mainly at the episode or trajectory level, which can diagnose a completed failure but cannot govern the physical execution while it unfolds~\cite{shinn2023reflexion,liu2023reflect,embodiskill2026,hong2026reflectiveplanning,feng2026procvlm}. Such post-hoc reflection has inherent limitations: agents cannot online test alternative actions to verify whether a reflection is correct, credit assignment over an entire trajectory is difficult, and retrospective analysis often lacks access to the precise state at the moment of failure. As a result, the experiences summarized after execution are difficult to reuse and provide limited support for effective learning. The experience adapts poorly to the changing real-world dynamics~\cite{weng2025temporalactionselection,julian2020neverstoplearning,chen2023adaptonthego}.

To address this challenge, the key idea of this work is to introduce \textbf{code-based critics that evolve online for closed-loop execution}, governing physical execution and triggering agentic intervention according to the changing dynamics of actions and environments. Building on this idea, we present \sys, a closed-loop embodied harness that self-evolves to scale physical intelligence (Figure~\ref{fig:teaser}).  The base policy models are frozen while evolving a harness $H=\{C,R,T\}$ of runtime critics, corresponding recovery skills from the rollouts. Specifically, we propose three different time-scale loops to enable self-evolution. First, a \emph{Critic-Governed Action Loop} executes learned critics at action frequency and invokes the corresponding recovery skills when necessary. Second, a \emph{Rollout-Batch Candidate Optimization Loop} clusters and diagnoses failures from each iteration, then proposes candidate critics and recoveries. Because skills and code provide no gradients, we draw on SkillOpt and EmbodiSkill~\cite{yang2026skillopt,embodiskill2026} to construct an SGD-like optimization process that makes bounded, stable updates in code space. Third, a \emph{Validation-Gated Skill Update Loop} admits only critic and recovery candidates that improve success rate and generalize across rollouts, and then adds them to the skill memory. The first loop enables closed-loop execution, while the second and third loops realize self-evolution.

The closed-loop enables the harness learning from self-exploration. This learning process also makes rollout throughput the rate limiter of intelligence scaling: the environment is the source of learning data, so faster rollouts produce faster evolution. We therefore propose and realize Z-Infra, to our knowledge the first rollout infrastructure designed specifically for self-evolving embodied agents. It decouples agent logic from heterogeneous execution resources through independent environment and model worker pools, batched inference, model partitioning, and asynchronous scheduling. This design scales the same agent across machines, accelerators, models, and environments without binding its logic to a particular hardware configuration.

% Physical intelligence is advancing along two complementary paths in search of an effective scaling paradigm. The first scales end-to-end policy models, including vision-language-action models (VLAs) and world-action models (WAMs), learning from demonstration data~\cite{brohan2022rt1,brohan2023rt2,kim2024openvla,black2024pi0,black2025pi05,bjorck2025groot,li2024cogact,bu2025univla,pertsch2025fast,dreamzero2026,cosmospolicy2026,fastwam2026,yu2026wall,team2026xiaomi,lingbot_va,lingbot_vla,qwen_vla,qwen_robotmanip}.
% \xiangyu{Learning from demonstration data? (vs. learning from exploration, assisted by frontier models / foundation models.)}
% However, embodied data remain scarce, and models trained on limited data distributions are brittle under the changing dynamics of real-world deployment; the gap from demonstration to reliable real-world execution therefore remains open.
% The second path uses large language models as embodied agents to orchestrate policy models, code, tools, and control primitives, as explored by CaP-X, ASPIRE, EnPIRE, Claude for Robotics, and HarnessVLA~\cite{capx2026,aspire2026,xiao2026enpire,anthropic2026clauderobotics,zhang2026harnessvla}, learning from self exploration. These systems alleviate limitations of end-to-end policies, but the harness must itself adapt to the dynamic deployment environment. Existing harnesses remain static and open-loop, and their agents follow fixed skills rather than learning continuously from accumulated experience. This work enables the scaling of embodied agent harnesses through self-evolution: as rollout experience increases, the harness continues to improve.
% \xiangyu{See latex comments for citation candidates, select suitable ones, add to correct place.}
% % TODO, Let agent add citations, look for existing item in .bib before looking it up in web, cross-check them with web.
% % Models (cite them by VLA and WAM separately is better: wall-oss-0.5, rldx, galexea g0.5, xiaomi-robotics-1, x-vla, qwen-robotmanip, cosmos3, fast-wam, x-wam, lingbot-va.
% % Datasets: DROID, Open X Embodiment,
% % limitation of learning e2e policy from demonstration data:
% % 1. **Data Quality in Imitation Learning**
% % 3. **A Reduction of Imitation Learning and Structured Prediction to No-Regret Online Learning**
% % 4. **KitchenShift: Evaluating Zero-Shot Generalization of Imitation-Based Policy Learning Under Domain Shifts**
% % 5. **Learning to Adapt in Dynamic, Real-World Environments Through Meta-Reinforcement Learning**
% % 6. **What Matters in Learning from Offline Human Demonstrations for Robot Manipulation**
% % 7. **The Pitfalls of Imitation Learning when Actions are Continuous**
% % 8. **Decomposing the Generalization Gap in Imitation Learning for Visual Robotic Manipulation** — quantifies policy sensitivity to different environmental variations in both simulation and real-robot experiments. ([arxiv.org](https://arxiv.org/abs/2307.03659?utm_source=openai))

% The evolving of embodied agents is fundamentally bottlenecked by the high-frequency interaction of the robots and the changing environment~\cite{li2025holdbeerlearninggentle,lee2022realtimemodelpredictivecontrol}. 
% Physical tasks require decisions to remain tightly coupled to the current robot and environment state, often changing within a millisecond-level latency budget~\cite{sinha2024realtime,pertsch2025fast}. 
% Large agentic models cannot make decisions at this frequency in real-world systems~\cite{yan2026actingunderstandingasynchronoussemanticaction,zhang2025hirtenhancingroboticcontrol,tan2024fouriercontrollernetworksrealtime,ding2025streammind,zheng2026emgardeproposematchframeworkproactive}. 
% Existing methods~\cite{huang2026actprobeactionspaceprobeearly,shinn2023reflexion,wang2026eeagent,embodiskill2026,zhang2026resync} therefore perform reflection mainly at the episode or trajectory level, which can diagnose a completed failure but cannot govern the physical execution while it unfolds. Their static trajectory skills also adapt poorly to changing real-world dynamics.
% % \xiangyu{See latex comments for citation candidates, select suitable ones, add to correct place.}
% % TODO, Let agent add citations, look for existing item in .bib before looking it up in web, cross-check them with web.
% % Physical control requires high-frequency state-feedback loops: 1. EvoControl: Multi-Frequency Bi-Level Control for High-Frequency Continuous Control. 2. Hold My Beer: Learning Gentle Humanoid Locomotion and End-Effector Stabilization Control 3. Real-Time Model Predictive Control for Industrial Manipulators with Singularity-Tolerant Hierarchical Task Control
% % Large VLM/VLA models have too much latency for direct high-frequency control: 1. HiRT: Enhancing Robotic Control with Hierarchical Robot Transformers 2. Acting While Understanding: Asynchronous Semantic-Action Decoupling for Real-Time Vision-Language-Action Models 3. Fourier Controller Networks for Real-Time Decision-Making in Embodied Learning
% % Existing reflection is often performed after a trial, episode, or trajectory; Post-hoc reflection can diagnose failures but does not provide low-level execution-time governance: 1. Reflexion: Language Agents with Verbal Reinforcement Learning. 2. REFLECT: Summarizing Robot Experiences for Failure Explanation and Correction. 3. EmbodiSkill: Skill-Aware Reflection for Self-Evolving Embodied Agents. 4. Learning from Trials and Errors: Reflective Test-Time Planning for Embodied LLMs. 5. ProcVLM: Learning Procedure-Grounded Progress Rewards for Robotic Manipulation
% % Other: Temporal Action Selection for Action Chunking; Never Stop Learning: The Effectiveness of Fine-Tuning in Robotic Reinforcement Learning; Adapt On-the-Go: Behavior Modulation for Single-Life Robot Deployment

% To solve this, the key insight of this work is to evolve the code-based critics online, governing the execution, to enable the closed-loop execution. Around that, we present \sys, a closed-loop embodied harness for self-evolving physical intelligence (Figure~\ref{fig:teaser}).  The base policy models are frozen while evolving a harness $H=\{C,R,T\}$ of runtime critics, corresponding recovery skills from the rollouts (Figure~\ref{fig:teaser}). Specifically, we propose the three loops to enable the self-evolving. First, a \emph{Critic-Governed Action Loop} executes learned critics at action frequency and invokes the corresponding recovery skills when necessary. Second, a \emph{Rollout-Batch Candidate Optimization Loop} clusters and diagnoses failures from each iteration, then proposes candidate critics and recoveries. Because skills and code provide no gradients, we draw on SkillOpt~\cite{yang2026skillopt} and EmbodiSkill~\cite{embodiskill2026} to construct an SGD-like optimization process that makes bounded, stable updates in code space. Third, a \emph{Validation-Gated Skill Update Loop} admits only critic and recovery candidates that improve success rate and generalize across rollouts, and then adds them to the skill memory.

% The three loops enable harness self-evolution, but they also make rollout throughput the rate limiter of intelligence scaling: the environment is the source of learning data, so faster rollouts produce faster evolution. We therefore propose and realize Z-Infra, to our knowledge the first rollout infrastructure designed specifically for self-evolving embodied agents. It decouples agent logic from heterogeneous execution resources through independent environment and model worker pools, batched inference, model partitioning, and asynchronous scheduling. This design scales the same agent across machines, accelerators, models, and environments without binding its logic to a particular hardware configuration.

Our main results are:
\begin{itemize}
%   \item \sys achieves state-of-the-art task success, improving over the
% strongest comparable HarnessVLA baseline by 20.3\% on
% LIBERO-Pro (90.8\% vs. 70.5\%) and 2.0\% on RoboCasa
% (93.6\% vs. 91.6\%).
\item Under our current rollout budget, \sys achieves state-of-the-art task success, substantially improving over current policy models and embodied-agent baselines: 90.8\% on LIBERO-Pro and 93.6\% on RoboCasa. Since performance continues to improve across evolution rounds, further rollout experience is expected to yield additional gains.
\item Success scales with evolution iterations: success increases from 34.5\% to 90.8\% on
LIBERO-Pro and from 73.6\% to 93.6\% on RoboCasa within several evolution iterations. 
\item The learned skills demonstrate zero-shot transfer capability to similar tasks. Take the PnP-Stove task in RoboCasa as an example, the pregrasp, regrasp, and stable-placement skills learned during the evolution of
transfer zero-shot to three related PnP tasks without target-specific
optimization: success improves from 58\% to 82\% on PnP-Sink, from 62\% to
80\% on PnP-Cabinet, and from 72\% to 90\% on PnP-Toaster.
\item We observe clear ``aha moments'' in which success remains low during
early evolution rounds but rises abruptly once the agent discovers the key
critic--recovery mechanism: for example, from 15\% to 95\% on Wine Bottle in Bowl and from
5\% to 90\% on Put Cream Cheese on Bowl.
  \item The \sys inference latency decreases by 91\% compared to RPent, i.e., an $11.1\times$ speedup. 
  \item Z-Infra increases valid rollout throughput from 1.7 to 35.1 episodes/min, a 20.6$\times$ improvement, directly accelerating the harness evolution loop.
\end{itemize}

Our contributions are: 
\begin{itemize}
  \item The first to realize a self-evolving embodied agent through learnable code-based critics and three coordinated evolution loops operating at action, rollout-batch, and iteration timescales.
  \item The first infrastructure designed to support embodied-agent self-evolution, decoupling agent logic from heterogeneous hardware resources for scalable rollout generation and execution.
  \item We demonstrate the scaling capability of the embodied harness: with increasing rollout and evolution iterations, it progressively improves task success to SOTA among existing models or embodied agents.
\end{itemize}


% \ting{Update intro as discussed: scaling important -> self-evolve challenge/How to realize -> scaling, aha -> contribution}

% Physical intelligence is advancing along two complementary paths. The first scales end-to-end foundation policies, including vision-language-action models, to acquire broad manipulation priors from increasingly diverse robot data~\cite{brohan2022rt1,brohan2023rt2,kim2024openvla,black2024pi0,black2025pi05}. 
% \xiangyu{Why VLA only? Maybe Vision-Language-Action Models (VLAs) [rt-1, rt2, openvla, pi0, pi0.5, gr00t, wall-oss, rldx, galexea, xiaomi, qwen] and World Action Models (WAMs) [cosmos policy, cosmos3, fast-wam, x-wam, lingbot, ...]?}
% Despite their rapid progress, these models remain constrained by expensive embodied data, deployment-time distribution shift, and errors that compound over long horizons \xiangyu{need citations (e.g., evaluation / benchmark) to support each point (I'm sure there are)}. The second path builds embodied agents and harnesses that compose foundation models, code, planners, memory, perception and action modules, and external tools into complete task-solving systems~\cite{driess2023palme,liang2023codeaspolicies,anthropic2026clauderobotics,zhang2026harnessvla}.
% \xiangyu{+ Cap-X?}
% A VLA \xiangyu{An end-to-end policy model?} is therefore one possible capability exposed to an agent, rather than a necessary substrate for every embodied harness. However, most existing harnesses are optimized to complete the current episode; their execution logic and skills remain largely static across repeated deployment.

% Static execution is insufficient for physical intelligence operating in open-ended environments. Pretraining can teach broad physical laws and reusable priors, but deployment-time self-evolution is needed to acquire the local ``vocabulary'' of a workspace: its recurring failure signatures, operational conventions, and effective recovery strategies. Recent embodied systems have begun to improve policies or data during deployment~\cite{xiao2026enpire,li2025veritas,agibot2026lwd}, \xiangyu{what about offline RL works like RECAP STEAM?} discover reusable skills and programs~\cite{aspire2026,zhang2026resync,embodiskill2026}, or adapt behavior at test time~\cite{robottt2026,wang2026eeagent}. These efforts establish important components of self-improvement, but typically optimize a particular policy, memory, or skill mechanism in isolation. They do not yet provide an integrated loop that combines governed execution, stable optimization of external skills, and rollout infrastructure capable of sustaining improvement at scale.

% Self-evolving digital agents offer a useful starting point: systems such as Reflexion, Self-Refine, Voyager, and OPRO improve behavior through feedback, memory, program synthesis, or iterative optimization~\cite{shinn2023reflexion,madaan2023selfrefine,wang2023voyager,yang2024opro}. \xiangyu{I didn't follow much but what about recent agent/RSI works? these works are tooo old (2024 and before)!}
% Their assumptions, however, do not transfer directly to physical interaction. Digital actions are often discrete, inexpensive, reversible, exactly logged, and easy to evaluate, whereas embodied tasks involve continuous state, partial observability, contact dynamics, long-horizon error propagation, and potentially irreversible failures \xiangyu{also need citation support here}. Moreover, embodied execution models often generalize poorly under environmental shift and remain brittle when composed over long horizons. The harness is therefore not merely an auxiliary layer: through observation, tool selection, verification, intervention, and recovery, it can determine the effective end-to-end capability of the deployed system.

% Realizing deployment-time self-evolution raises three challenges. First, \emph{task-level success rewards are too sparse and too late}: they cannot prevent an early local error from propagating through the remainder of a trajectory. More frequent supervision is needed, yet existing critics are often large language or vision-language models, complex verifiers, or other costly procedures that cannot be invoked at every action step and across large rollout batches \xiangyu{cite existing methods}; consequently, most harnesses rely on terminal reflection or sparse checkpoints. Second, external critic and recovery skills must improve without destabilizing behavior: a plausible update may fix one failure mode while introducing regressions elsewhere, calling for optimization at action, rollout-batch, and iteration timescales with explicit acceptance gates. Third, the rate of intelligence improvement is bounded by the rate of informative rollouts. Embodied rollouts combine CPU-heavy simulation, GPU-heavy policy inference, perception and tool calls, environment resets, and irregular agent control flow, so tightly coupling agents to particular hardware leaves resources idle and slows the learning loop.
% \xiangyu{I think the 3 challenges need emphasize: be concise, clear, and orthogonal. E.g., sparse rewards in long-horizon rollouts (data efficiency); instable updates of external critic and recovery skills (learning stability); heterogeneous resource demands within evolution loops (infra complexity). If we could connect these 3 points logically it'll be even better.}

% We present \sys, a closed-loop embodied harness for self-evolving physical intelligence (Figure~\ref{fig:teaser}). In our VLA-centric instantiation \xiangyu{are we tied to VLA? what is VLA-centric?}, the base policy remains frozen while an evolvable harness $H=\{C,R,T\}$ maintains runtime critics, recovery skills, and tools under a fixed Orchestrator Agent. A \emph{Critic-Governed Action Loop} invokes efficient, grounded critics at action frequency and triggers recovery before local errors become terminal failures. Within each iteration, a \emph{Rollout-Batch Candidate Optimization Loop} diagnoses clustered failures, samples alternative critic and recovery candidates, and evaluates their causal effect over fresh rollouts; a \emph{Validation-Gated Skill Update Loop} then admits only candidates that improve held-out success, producing gradual and non-regressive harness updates. Beneath these loops, Z-Infra decouples agent logic from heterogeneous execution resources through independent environment and model worker pools, batched inference, model partitioning, and asynchronous scheduling. Together, these mechanisms turn rollout experience into verified, reusable execution skills while preserving a stable foundation policy.

% We evaluate \sys on LIBERO~\cite{liu2023libero} and RoboCasa~\cite{nasiriany2024robocasa} along four dimensions. First, it achieves state-of-the-art task success by augmenting a fixed execution model with learned critic and recovery skills. Second, success scales consistently with additional evolution iterations, demonstrating that repeated deployment produces cumulative capability rather than isolated episode-level reflection. Third, recovered skills transfer across related tasks, showing that the harness captures reusable failure mechanisms rather than memorizing individual trajectories. Finally, the decoupled rollout system substantially increases rollout throughput and reduces agent inference latency relative to the coupled baseline. \ting{Insert the final LIBERO/RoboCasa accuracy gains, rollout-throughput gain, and inference-latency reduction.}

% A closer examination of the scaling curves reveals an \emph{aha moment}: in one representative task, success rises abruptly from approximately $5\%$ to $100\%$ after the rollout budget crosses a critical point. Because the underlying execution model is frozen, this transition cannot be attributed to a weight update in the policy. Instead, sufficient rollout coverage exposes a dominant long-horizon bottleneck, after which candidate optimization discovers and validates the critic--recovery pair that resolves it. Correcting that single critical milestone moves many trajectories across the task-success boundary, producing a discrete capability acquisition within an otherwise gradual, gated optimization process. This finding connects the algorithmic and systems contributions: rollout scale is not only an efficiency metric, but also determines the evidence coverage and search opportunity required to discover capability-changing skills.

% \ting{I have one question for our scaling. Can we answer what is the bound? like after more iterations, can we make the tasks SR all > 90\% (which means production-level ready)? Or the scaling has a bound by VLA/WAM, which requires some kind of immitation learning}






==> arxiv_submission/tex/method.tex <==
% \section{Overall Design}
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.98\linewidth]{figs/overall-design.pdf}
%   \caption{Overall design of the self-evolving agent and rollout infrastructure. split agent @dingxin and infra @miliang}
%   \label{fig:overall-design}
% \end{figure}

% \subsection{Self-evolving Embodied Harness}
% \paragraph{Problem formulation}
% @dingxin
% Key challenges/bottlenecks of current embodied agents:
% - The agent enables the planning->execution->reflection->self evolve loop

%   - Different-frequency reflection, from task level to action level.
%   - Learnable skills for continuous improvement
%   - Expendable toolsets
%   - High-frequency critic rather than final reward only

\section{Enabling Deployment-Time Evolution of Embodied Agents}
\subsection{Problem Formulation: Dual-Agent Governance and Evolutionary Architecture}
\label{sec:problem}
We formalize the long-horizon robotic manipulation task as an authority-constrained governance and evolution process. The framework incorporates an online \textbf{Orchestrator Agent} for adjudication and offline \textbf{Evolutionary Agents} for optimization, enabling closed-loop capability evolution without altering the underlying policy parameters.

\subsubsection{Fixed Runtime Components}
The execution is driven by two core entities whose internal parameters and logic remain invariant throughout the evolution:
\begin{enumerate}
    \item \textbf{Action Policy ($\pi$)}: Given observation $s_t$ and goal $g$, it generates low-level actions $a_t = \pi(s_t, g; \theta)$, where parameters $\theta$ satisfy the constraint $\nabla \theta = 0$.
    \item \textbf{Orchestrator Agent ($\mathcal{A}_{orch}$)}: Acting as a fixed multimodal reasoning operator \cite{anthropic2025claudesonnet45,openai2026gpt55,openai2026gpt56}, $\mathcal{A}_{orch}$ functions as a high-level commander responsible for auditing real-time evidence and approving mode transitions. Its decision logic remains constant during evolution.
\end{enumerate}

\subsubsection{Evolvable Harness ($\mathcal{H}$)}
The Harness $\mathcal{H}$ is the target of the evolutionary process, providing $\mathcal{A}_{orch}$ with means to perceive and intervene in the environment. We define it as:
\begin{equation}
    \mathcal{H} = \{C, R, \mathcal{T}\}
\end{equation}
\begin{itemize}
    \item \textbf{Runtime Critic ($C$)}: A set of \textbf{high-frequency} monitoring functions that persistently scan the trajectory $\tau_{0:t}$ to generate a \textbf{structured proposal} $P_t$:
    \begin{equation}
        P_t = C(\tau_{0:t}) = \langle e_t, \hat{\sigma}_t \rangle
    \end{equation}
    where $e_t$ represents auditable evidence of failure (e.g., collisions, stalled progress) and $\hat{\sigma}_t$ is the suggested execution mode.
    \item \textbf{Recovery Playbook ($R$)}: A structured library of strategies mapped to specific causal failure mechanisms, providing actionable options for adjudication.
    \item \textbf{Heterogeneous Toolset ($\mathcal{T}$)}: A collection of executable tools and operators (e.g., planners, grasp detectors, recovery modules)\cite{zucker2013chomp, sundermeyer2021contact,kirillov2023segment} that can be generated, instantiated, selected, and refined during evolution. The toolset evolves to satisfy the monitoring requirements of $C$ and the recovery logic of $R$, enabling the harness to acquire and adapt its execution capabilities rather than merely tuning parameters of predefined tools.
\end{itemize}

\subsubsection{Authority Hierarchy: Online Adjudication Logic}
During execution, the final operational mode $\sigma_t$ ($\sigma_t = 0$ for VLA or WAM, $\sigma_t > 0$ for specialized tools) is determined by the adjudication function:
\begin{equation}
    \sigma_t = \mathcal{A}_{orch}(P_t, R, \mathcal{T}, \mathcal{K})
\end{equation}
where $P_t$ is the real-time proposal from $C$, and $\mathcal{K}$ represents the \textbf{task knowledge context}, including pre-defined milestones, success criteria, and environmental constraints. This protocol enforces \textbf{evidence-driven decision-making}: although $C$ operates at a high frequency, an intervention is only permitted if the evidence $e_t$ is validated and accepted by $\mathcal{A}_{orch}$.

\subsubsection{Offline Optimization: Evolutionary Agents}
To optimize $\mathcal{H}$, we introduce \textbf{Evolutionary Agents} $\mathcal{A}_{evo}$ as the driving force for offline refinement. $\mathcal{A}_{evo}$ iteratively improves the harness components by analyzing the failed rollout data $\mathcal{D}_{fail}$:
\begin{equation}
    \mathcal{H}^{(k+1)} \leftarrow \mathcal{A}_{evo}(\mathcal{D}_{fail}^{(k)}, \mathcal{H}^{(k)})
\end{equation}
$\mathcal{A}_{evo}$ extracts causal mechanisms from failure evidence, generates repair patches, and abstracts local experiences into versioned harness. It modifies the runtime behavior of $\mathcal{A}_{orch}$ by restructuring its available sensing ($C$) and action ($R, \mathcal{T}$) space.

\paragraph{Optimization Objective}
The ultimate goal of Zetta is to find the optimal configuration $\mathcal{H}^*$ that maximizes the expected task success rate $J$ while keeping $\pi_{VLA}$ and $\mathcal{A}_{orch}$ invariant:
\begin{equation}
    \max_{\mathcal{H}} J(\mathcal{H}) = \mathbb{E}_{g, s_0 \sim \mathcal{D}} \left[ \text{Success}(\tau) \mid \pi, \mathcal{A}_{orch}, \mathcal{H} \right]
\end{equation}




\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figs/agent_framework_v2.pdf}
 \caption{\textbf{Overview of the Zetta evolutionary framework.} The system operates in a continuous loop between online execution and offline evolution. \textbf{(Left) Parallel Rollouts:} Action policy executes tasks, monitored by an \textit{Evolvable Harness} ($\mathcal{H}$) composed of Critics ($C$), Recovery ($R$), and Tools ($T$), all under the high-level adjudication of an \textit{Orchestrator Agent}. Rollouts are categorized into success and failure trajectories. \textbf{(Right) Reflection \& Evolve:} Failed trajectories trigger a three-phase offline evolution cycle. \textit{Phase I} profiles failures by clustering them against successful reference baselines. \textit{Phase II} performs causal diagnosis to locate the root failure layer ($L^*$), followed by minimal harness repair to update $C$, $R$, and $T$. \textit{Phase III} generalizes seed-specific repairs into a unified, versioned \textit{Harness Package} ($\mathcal{H}_{merged}$), which is then fed back into the execution loop.}
    \label{fig:Zetta_overview}
\end{figure}

\subsection{System Challenges and Design Principles}

To address the limitations of current embodied AI systems based on frozen Vision-Language-Action (VLA) policies, we identify three core challenges that motivate the design of the Zetta framework.

\paragraph{Challenge 1: The Open-Loop Semantics-Physics Gap in Frozen Foundation Models.}
SOTA VLA/WAM models possess strong semantic understanding but operate as \textbf{open-loop} feedforward policies during inference \cite{black2025pi05,bjorck2025groot,li2026lingbotva,fastwam2026}. They lack closed-loop sensory-motor perception to correct physical execution errors (e.g., object slippage, minor collisions) in real-time. Consequently, minor disturbances often cascade into total task failure because the policy cannot monitor or adjust to its own physical state.

\noindent \textbf{Zetta Design Principle: High-Frequency State Governance.} We augment the frozen VLA/WAM with decoupled, \textbf{high-frequency runtime critics ($C$)}. Operating above the action policy's  inference rate, these critics continuously monitor the physical execution state and trigger interventions at the earliest signs of deviation from the nominal distribution, transforming the system into a closed-loop governance paradigm.



\paragraph{Challenge 2: The Generalization Pitfall of Over-Parameterized Repair.}
Determining the root cause of physical failures is complex. Ad-hoc debugging often leads to "overfitting" repairs—adjusting low-level control parameters to force success on a specific failure instance \cite{muratore2022robot,tan2018sim,rana2023bayesian}. While resolving the immediate fault, such modifications corrupt the action distribution essential for the VLA's semantic generalization, causing severe performance degradation on unseen held-out seeds, thus sacrificing global generalizability.

\noindent \textbf{Zetta Design Principle: Hierarchical Causal Diagnosis for Minimal Intervention.} We implement a strict \textbf{Top-Down Hierarchical Causal Diagnosis} logic. The Diagnosis Agent $\mathcal{A}_{diag}$ traverses layers in priority order: from $Evaluation \to Critic \to State \to Planning \to Recovery \to Parameter$.\cite{pettersson2005execution,donald1988geometric,gu2026safe} Adhering to the principle that ``if high-level logic resolves the failure, never modify low-level parameters,'' ensures patches are applied at the minimal effective layer, preserving the foundation model's integrity.

\paragraph{Challenge 3: The Scalability of Expert-in-the-Loop Debugging.}
Relying on human experts to manually analyze and patch every individual failure instance across long-tail task distributions is expensive and fundamentally unscalable \cite{hu2026rac,zhu2026beyond,li2025hamster,liu2024moka}. This approach cannot keep up with the infinite variations of initial conditions inherent in general-purpose manipulation.

\noindent \textbf{Zetta Design Principle: Automated Evolutionary Generalization.} We replace manual debugging with a \textbf{fully automated evolutionary learning loop (Loop 1-3)}. The Evolutionary Agent $\mathcal{A}_{evo}$ autonomously abstracts seed-specific failures into generalized harness based on \textit{task invariants}. Furthermore, an enforced \textbf{Held-out Generalization Protocol} validates consolidated harness on strictly isolated test sets, enabling automated scaling of robust governance strategies.







\subsection{Phase I: Empirical Failure Profiling and Baseline Establishment (Loop 1)}

At the onset of the evolutionary cycle, we conduct large-scale sampling of the Action policy $\pi$ across a predefined development seed set $\mathcal{D}_{dev}$. The objective is to establish a performance baseline through pure VLA closed-loop execution without governance intervention. The resulting raw corpus is defined as $\mathcal{B}_{raw} = \{ \tau^{(j)} \mid seed_j \in \mathcal{D}_{dev} \}$.

\paragraph{Deterministic Scheduling and Execution Protocol}
To ensure empirical rigor and reproducibility, Loop 1 enforces strict infrastructure management through two deterministic dimensions:
\begin{itemize}
    \item \textbf{Deterministic Routing}: All rollout tasks are dispatched via a centralized resource scheduler. The scheduler routes tasks based on real-time loads and memory thresholds of computation nodes (e.g., 4090 GPU pools). This mechanism ensures that all rollouts within a batch run under identical software containers, simulator versions, and hardware configurations, eliminating observational noise from environmental heterogeneity.
    \item \textbf{Validity Determination and Isolation}: The system explicitly distinguishes between \textit{infrastructure failure} and \textit{policy failure}. We define a validity function $\text{Valid}(seed_j) \in \{True, False\}$. A rollout is included in the \textbf{valid rollout set $\mathcal{V}$} only if it completes with a full trace of sensor data and video evidence:
    \begin{equation}
        \mathcal{V} = \{ seed_j \in \mathcal{D}_{dev} \mid \text{Valid}(seed_j) = True \}
    \end{equation}
    For infrastructure-invalid attempts (e.g., network fluctuations, simulator crashes), a mandatory rerun policy is enforced using the original logical seeds until a valid trajectory is produced, ensuring the statistical distribution of $\mathcal{V}$ does not drift due to non-policy factors.
\end{itemize}

\paragraph{Multi-dimensional Evidence Acquisition}
For each valid rollout $\tau^{(j)} \in \mathcal{V}$, the system employs an \textbf{append-only} mode to preserve a comprehensive observational stream. A complete trajectory instance $\tau^{(j)}$ is represented as a multimodal time series:
\begin{equation}
    \tau^{(j)} = \{ (s_t, a_t, \mu_t, \phi_t) \}_{t=0}^T
\end{equation}
where $\mu_t$ denotes the completion status of task-specific semantic milestones, and $\phi_t$ captures physio-auxiliary signals such as collision intensities and contact force vectors.

\paragraph{Categorization and Indexing}
The resulting corpus is processed into two core repositories for the Evolutionary Agents $\mathcal{A}_{evo}$:
\begin{enumerate}
    \item \textbf{Successful Reference Index ($I_{succ}$)}: Successful trajectories $\mathcal{V}_{succ} \subset \mathcal{V}$ are aggregated by milestones:
    \begin{equation}
        I_{succ}(\mu) = \{ s_t \mid \tau \in \mathcal{V}_{succ}, \mu_t = \mu \}
    \end{equation}
    This index reveals the ``nominal distribution'' of task success, serving as a benchmark for identifying deviations.
    \item \textbf{Failed-Seed Manifest ($\mathcal{M}_{fail}$) and First Missing Milestone ($m^*$)}: All unsuccessful samples and their evidence chains are compiled into a manifest. To localize the task stage where failure occurred, we introduce the \textbf{First Missing Milestone ($m^*$)}.
    
    Given an ordered sequence of semantic milestones $M = \langle m_1, m_2, \dots, m_{goal} \rangle$, $m^*$ is defined as the first element in the sequence that was not observed in the trajectory history:
    \begin{equation}
        m^* = \min \{ m_k \in M \mid m_k \notin \{ \mu_t \}_{t=0}^T \}
    \end{equation}
    The introduction of $m^*$ serves two purposes: providing a coarse-grained clustering criterion for failures and narrowing the search space for causal diagnosis by focusing $\mathcal{A}_{diag}$ on the evidence during the transition from $m^*-1$ to $m^*$.
\end{enumerate}






\noindent \textbf{The Evolution Cycle: From Data to Harness.} Based on the formalization of the Evolutionary Agent $\mathcal{A}_{evo}$ in Section \ref{sec:problem}, the operational logic is realized through a tripartite pipeline: \textbf{Diagnosis} ($\mathcal{A}_{diag}$), \textbf{Repair} ($\mathcal{A}_{repr}$), and \textbf{Generalization} ($\mathcal{A}_{gen}$). This structure ensures the systematic extraction of causal knowledge from the raw failure corpus $\mathcal{M}_{fail}$. As the pipeline's starting point, the primary mission of $\mathcal{A}_{diag}$ is to identify the root causal mechanisms of failures.

\subsection{Phase II Stage 1: Failure Clustering and Causal Diagnosis}

\subsubsection{Mechanism-Level Failure Clustering and Medoid Seed Selection}
The diagnosis begins with a structural analysis of the Failed-Seed Manifest $\mathcal{M}_{fail}$ produced in Loop 1. Instead of superficial categorization based on final outcomes, $\mathcal{A}_{diag}$ clusters seeds based on the \textbf{Earliest Observable Divergence (EOD)}. We define $t_{EOD}$ as the first time step in a trajectory $\tau \in \mathcal{M}_{fail}$ where the state distribution deviates from the ``healthy'' distribution described by $I_{succ}$:
\begin{equation}
    t_{EOD} = \min \{ t \mid \text{dist}(s_t, s_t^{ref}) > \epsilon, s_t^{ref} \in I_{succ}(\mu_t) \}
\end{equation}
where $\text{dist}(\cdot)$ is a state-space distance metric and $\epsilon$ is a predefined threshold. 

Utilizing $t_{EOD}$ and its context—including the first missing milestone $m^*$, robot-object relative poses, and active tool IDs—$\mathcal{A}_{diag}$ partitions $\mathcal{M}_{fail}$ into mutually exclusive clusters $\mathcal{K} = \{K_1, K_2, \dots, K_n\}$, where each $K_i \subseteq \mathcal{M}_{fail}$ contains seeds sharing similar failure signatures. To reduce computational overhead and extract mechanism invariants, a \textbf{medoid seed} $seed_{med} \in K_i$ is selected for each cluster. Defined as the sample closest to the cluster center in the feature space, $seed_{med}$ serves as the primary subject for in-depth causal diagnosis.

\paragraph{Single-View Grounded Observation Protocol}
To eliminate spatial reasoning inconsistencies and multiview hallucinations \cite{wu2026grounded,dongfang2026multimodal,huang2022inner} in multimodal models, $\mathcal{A}_{diag}$ adheres to a strict \textbf{single-view grounded protocol}:
\begin{itemize}
    \item \textbf{Primary View Selection}: The agent must first designate a primary view from available video streams, defined as the angle that most clearly exhibits the end-effector, the target object, and the critical contact interface.
    \item \textbf{Evidence Consistency}: Once the primary view is established, all visual reasoning throughout the diagnosis must be anchored to it. If the primary view provides insufficient evidence, the system is mandated to revert to internal simulator states, sensor trajectories, and physical signals $\phi_t$ for cross-modal verification, rather than switching viewpoints, ensuring spatial-logical consistency.
\end{itemize}

\subsubsection{Top-Down Hierarchical Causal Diagnosis}
For the selected $seed_{med}$, $\mathcal{A}_{diag}$ executes a systematic top-down inspection logic across the diagnostic layer space $\mathcal{L} = \{L_{eval}, L_{crit}, L_{state}, L_{plan}, L_{recv}, L_{param}\}$. The task is to localize the root cause by finding the highest-priority layer $L^*$ such that:
\begin{equation}
    L^* = \text{arg max}_{L \in \mathcal{L}} \{ \text{IsRootCause}(L) \mid \text{Evidence from } \tau, \text{Primary View} \}
\end{equation}
The inspection order follows the hierarchical priority:
\begin{enumerate}
    \item \textbf{Evaluation Layer ($L_{eval}$)}: Check for errors in success criteria or milestone progress logic.
    \item \textbf{Critic Layer ($L_{crit}$)}: Determine if runtime critics $C$ exhibit false negatives or false positives.
    \item \textbf{State Representation Layer ($L_{state}$)}: Verify if object poses or contact information deviated from physical ground truth.
    \item \textbf{Planning/Control Layer ($L_{plan}$)}: Analyze if the VLA policy or tools failed to handle physical constraints despite correct states.
    \item \textbf{Recovery Layer ($L_{recv}$)}: If the failure occurred during recovery, check for flaws in the playbook logic.
    \item \textbf{Parameter Layer ($L_{param}$)}: Inspect specific control gains or action thresholds.
\end{enumerate}

\textbf{Cluster Consistency and Repair Specification}
Upon determining $L^*$ for $seed_{med}$, $\mathcal{A}_{diag}$ verifies the mechanism's consistency across other members of $K_i$. Finally, the agent outputs a \textbf{Repair Candidate Specification} for each validated mechanism, detailing the localized layer, the causal evidence chain, and functional requirements for updating the harness components ($C, R, \mathcal{T}$).




\subsection{Phase II Stage 2: Critic-Guided Harness Repair and Validation}
\label{sec:phase_ii_stage_2}

This stage is led by the Repair Agent $\mathcal{A}_{repr}$, whose objective is to implement a minimal harness patch $\mathcal{H}_{patch} = \{C^*, R^*, \mathcal{T}^*\}$ that resolves the specific root layer $L^*$ identified during diagnosis, while strictly preserving the integrity of the base Action Policy $\pi$.

\subsubsection{Harness Component Instantiation and Re-entry Logic}
$\mathcal{A}_{repr}$ begins by instantiating the requisite governance components dictated by the diagnostic specification. This entails targeted updates across the harness:
\begin{itemize}
    \item \textbf{Critic Enhancement ($C^*$)}: Development or refinement of high-frequency monitoring functions designed to detect the specific precursor conditions of the failure, generating structured proposals $P_t$ upon deviation.
    \item \textbf{Recovery Drafting ($R^*$) and Tool Adaptation ($\mathcal{T}^*$)}: Definition of actionable recovery playbooks and the adaptation or synthesis of executable tools to address the causal failure mechanism.
\end{itemize}

Crucially, to \textbf{ensure safe and seamless integration}, $\mathcal{A}_{repr}$ embeds a strict \textbf{VLA Re-entry Contract} within the recovery logic of $R^*$ and $\mathcal{T}^*$. This contract defines the logical predicate $\Psi(s_t)$ that dictates when control is relinquished back to the base policy $\pi_{VLA}$. Control handover is permitted only if the original failure evidence $e_t$ is explicitly cleared and the physical state has reached equilibrium, as defined by stable contact forces. We define this predicate as:
\begin{equation}
    \Psi(s_t) = \mathbb{1}(\text{FailureCleared}) \land \mathbb{1}(\text{Stability}(s_t) > \gamma)
\end{equation}
where the \textbf{Failure Cleared} term is a boolean function verifying that the specific conditions constituting evidence $e_t$ (e.g., collision risk or pose deviation) have been fully resolved by the recovery actions. Simultaneously, the \textbf{Stable Contacts} term evaluates physio-auxiliary signals $\phi_t$ to ensure the connection between the robot and the object has reached a physical equilibrium. Specifically, $\text{Stability}(s_t)$ measures the magnitude of contact torque oscillations and grasp forces, while $\gamma$ is a stability threshold ensuring safe takeover by the VLA, preventing secondary failures due to transient dynamic effects. This contract acts as a crucial safeguard, preventing instability from triggering secondary failures upon policy resumption.

\subsubsection{Closed-Loop Validation Protocol and Success Criteria}
Following implementation, the patch $\mathcal{H}_{patch}$ undergoes a rigorous two-step closed-loop validation on the original medoid seed. First, a \textit{diagnostic replay} confirms that the enhanced critic $C^*$ now correctly identifies the divergence point $t_{EOD}$. Second, a \textit{fresh closed-loop rollout} is executed from the initial state. A repair patch is only considered validated and successfully \textit{passed} if the task reaches the goal milestone and all interventions are properly adjudicated by $\mathcal{A}_{orch}$ in compliance with the re-entry contract:
\begin{equation}
    \text{Success}(\mathcal{H}_{patch}) = \mathbb{1}(\mu_{T, new} = m_{goal} \land \forall t \in \text{Intv}, \text{Adjudicated by } \mathcal{A}_{orch})
\end{equation}
where $\mu_{T, new}$ is the final milestone of the new trajectory and $\text{Intv}$ represents the intervention interval. Validated patches, along with their evidence, are then submitted to $\mathcal{A}_{gen}$ for multi-seed consolidation.


% \subsection{Phase II Stage 2: Critic-Guided Harness Repair and Validation }

% This stage is led by the Repair Agent $\mathcal{A}_{repr}$, whose objective is to implement a minimal harness patch $\mathcal{H}_{patch}$ addressing the identified root layer $L^*$ and validate its efficacy in a controlled closed-loop environment.

% \subsubsection{Harness Component Instantiation}
% $\mathcal{A}_{repr}$ receives the specification from the diagnosis phase and performs targeted updates on the harness components. We define the generated local patch as:
% \begin{equation}
%     \mathcal{H}_{patch} = \{C^*, R^*, \mathcal{T}^*\}
% \end{equation}
% The implementation logic is as follows:
% \begin{itemize}
%     \item \textbf{Critic Enhancement ($C^*$)}: If the root cause is localized at the critic layer ($L_{crit}$), $\mathcal{A}_{repr}$ develops or refines the high-frequency monitoring functions. The updated critic must accurately capture previously missed physical anomalies and generate structured proposals $P_t$ containing causal evidence $e_t$.
%     \item \textbf{Recovery Drafting ($R^*$)}: Define or update recovery playbooks for the identified failure modes. Playbooks specify not only the candidate action sequences post-triggering but also the expected logic for returning from an intervention state to the nominal path.
%     \item \textbf{Tool Adaptation and Tuning ($\mathcal{T}^*$)}: Modify tool interfaces to meet recovery requirements or optimize tool execution parameters within physical constraints through sensitivity analysis, ensuring performance aligns with $R^*$.
% \end{itemize}

% \paragraph{The VLA Re-entry Contract}
% To ensure a seamless transition from manual intervention or tool execution back to the default VLA policy, $\mathcal{A}_{repr}$ embeds a strict \textbf{Re-entry Contract} within the patch. We define the re-entry logical predicate $\Psi(s_t)$, where control is handed back to $\pi_{VLA}$ only if $\Psi(s_t)$ is satisfied:

% \begin{equation}
%     \Psi(s_t) = \mathbb{1}(\text{FailureCleared}) \land \mathbb{1}(\text{Stability}(s_t) > \gamma)
% \end{equation}
% where:
% \begin{itemize}
%     \item \textbf{Failure Cleared}: A boolean function verifying that the original evidence $e_t$ (e.g., collision risk or pose deviation) has been explicitly resolved by the recovery actions.
%     \item \textbf{Stable Contacts}: This term evaluates physical signals $\phi_t$ to determine if the connection between the robot and the object has reached equilibrium. $\text{Stability}(s_t)$ measures the magnitude of contact torque oscillations and grasp forces, while $\gamma$ is a stability threshold ensuring safe takeover by the VLA, preventing secondary failures due to transient dynamics.
% \end{itemize}

% \subsubsection{Closed-Loop Validation Protocol and Success Criteria}
% The validation follows a rigorous two-step protocol to ensure the patch is effective in the original failure context ($seed_{med}$):
% \begin{enumerate}
%     \item \textbf{Diagnostic Replay}: The original failed trajectory from Loop 1 is fed into the updated critic $C^*$. The goal is to confirm whether it correctly triggers the expected proposal $P_t$ at or before the divergence point $t_{EOD}$.
%     \item \textbf{Fresh Closed-loop Rollout}: The task is re-executed under identical logical seeds and initial states. The success of this process is defined as:
%     \begin{equation}
%         \text{Success}(\mathcal{H}_{patch}) = \mathbb{1}(\mu_{T, new} = m_{goal} \land \forall t \in \text{Intv}, \text{Adjudicated by } \mathcal{A}_{orch})
%     \end{equation}
%     where $\mu_{T, new}$ is the final milestone of the new trajectory and $\text{Intv}$ represents the intervention interval. This requires that the task is completed and all deviations are explicitly approved by the Orchestrator.
% \end{enumerate}

% A repair patch is considered passed only if $seed_{med}$ successfully reaches the goal milestone in the closed-loop rollout and the re-entry contract $\Psi(s_t)$ is correctly invoked. Validated patches, along with their evidence, are then submitted to $\mathcal{A}_{gen}$ for multi-seed consolidation.


\subsection{Phase III: Harness Consolidation, Packaging and Generalization}
\label{sec:phase_iii}

In this final stage of the evolutionary cycle, the Generalization Agent $\mathcal{A}_{gen}$ transforms validated, seed-specific patches into a robust, unified governance harness. The objective is to abstract local repairs into mechanism-level invariants capable of resolving the entire failure cluster $K_i$, resulting in a versioned \textbf{merged harness $\mathcal{H}_{merged}$}.

\subsubsection{Mechanism Consolidation and Harness Packaging}
$\mathcal{A}_{gen}$ performs a cross-seed analysis to consolidate heterogeneous patches $\mathcal{H}_{patch, j}$ (for $seed_j \in K_i$) into a single, coherent configuration $\mathcal{H}_{merged} = \{C_{merged}, R_{merged}, \mathcal{T}_{merged}\}$. This process elevates governance logic from specific instances to general mechanisms and encapsulates it into a portable, standardized file structure.



The consolidation operator abstracts local experiences into task invariants:
\begin{itemize}
  \item \textbf{Critic Unification}: Individual monitoring functions are abstracted into a unified Critic $C_{merged}$. By applying logical OR operations on triggering conditions and dynamically adjusting noise thresholds, $C_{merged}$ ensures reliable failure detection across the diverse initial conditions present within the cluster.
    \item \textbf{Recovery Integration}: Seed-specific Recovery Playbooks are abstracted into $R_{merged}$, which generalizes action sequences to handle morphological variations of the same failure mode and standardizes the VLA Re-entry Contract $\Psi(s_t)$.
    \item \textbf{Toolset Expansion}: The Heterogeneous Toolset $\mathcal{T}_{merged}$ is expanded to include not only tuned existing operators but also \textbf{newly synthesized tools}. These executable scripts encapsulate specialized physical skills (e.g., high-precision impedance control) generated during the repair phase to address constraints beyond the base VLA's capabilities.
\end{itemize}
Mathematically, this consolidation is defined as:
\begin{equation}
    \mathcal{H}_{merged} = \text{Consolidate} \left( \{ \mathcal{H}_{patch, j} \mid seed_j \in K_i \} \right)
\end{equation}

To ensure the portability and version control of these evolved capabilities, $\mathcal{A}_{gen}$ externalizes the governance logic into a self-contained package, mapping components to distinct directories:
\begin{itemize}
    \item \textbf{$SKILL.md$}: Declares the high-level governance logic, including defined milestones $M$, Orchestrator adjudication rules, and the generalized re-entry predicate $\Psi(s_t)$.
    \item \textbf{$tools/$}: Contains the executable implementations and scripts for the evolved critics $C_{merged}$ and the toolset $\mathcal{T}_{merged}$.
    \item \textbf{$plans/$}: Stores the generalized recovery playbooks $R_{merged}$, mapping specific evidence to structured intervention strategies.
    \item \textbf{$params/$}: Holds the configuration files defining generalized numeric boundaries and thresholds for runtime execution.
\end{itemize}


\subsubsection{Rigorous Generalization Validation and Transition Protocol}
The final validated harness $\mathcal{H}_{merged}$ must satisfy stringent performance criteria via a dual-evaluation protocol to confirm genuine generalization.

\paragraph{Historical Regression and Held-Out Evaluation}
First, the harness undergoes **Historical Regression** testing, requiring it to successfully resolve all failed rollouts within the originating cluster $K_i$ with a 100\% success rate:
\begin{equation}
    \forall seed_j \in K_i, \text{Success}(seed_j \mid \mathcal{H}_{merged}) = 1
\end{equation}
Second, to confirm broader applicability, the harness is subjected to **Held-out Evaluation** on a strictly isolated dataset $\mathcal{D}_{held-out}$. The effectiveness of the evolution is quantified by the success rate increment $\Delta SR$ over the baseline VLA policy:
\begin{equation}
    \Delta SR = SR(\mathcal{D}_{held-out} \mid \mathcal{H}_{merged}) - SR(\mathcal{D}_{held-out} \mid \pi_{VLA})
\end{equation}

\paragraph{Dynamic Transition Protocol}
An evolutionary iteration is considered complete only when $\mathcal{H}_{merged}$ demonstrates robust performance on previously unseen data. If the evaluation on $\mathcal{D}_{held-out}$ reveals novel failure mechanisms that trigger modifications to $\mathcal{H}_{merged}$, the system enforces a strict data segregation policy. The original held-out seed is reclassified as a development seed ($\mathcal{D}_{dev} \leftarrow \mathcal{D}_{dev} \cup \{seed_{failed}\}$), and a fresh, previously unseen set must be selected for final validation before the iteration can be closed.

% \subsection{Phase III: Harness Generalization, Consolidation and Packaging}
% \label{sec:phase_iii}

% In this final stage of the evolutionary cycle, the Generalization Agent $\mathcal{A}_{gen}$ transforms validated, seed-specific patches into a robust, unified governance harness. The objective is to abstract local repairs into mechanism-level invariants capable of resolving the entire failure cluster $K_i$, resulting in a versioned \textbf{merged harness $\mathcal{A}_{merged}$}.

% \paragraph{Generalization and Consolidation Logic}
% $\mathcal{A}_{gen}$ performs a cross-seed analysis to consolidate heterogeneous patches $\mathcal{H}_{patch, j}$ (for $seed_j \in K_i$) into a single, coherent configuration $\mathcal{H}_{merged} = \{C_{merged}, R_{merged}, \mathcal{T}_{merged}\}$. This consolidation elevates governance logic from specific instances to general mechanisms:
% \begin{itemize}
%     \item \textbf{Critic Unification ($C_{merged}$)}: Individual monitoring functions are merged into a unified Critic $C_{merged}$. By applying logical OR operations on triggering conditions and decorrelating noise thresholds, $C_{merged}$ ensures reliable failure detection across the diverse initial conditions present in the cluster.
%     \item \textbf{Playbook Integration ($R_{merged}$)}: Seed-specific Recovery Playbooks are abstracted into $R_{merged}$, which generalizes action sequences to handle morphological variations of the same failure mode and standardizes the VLA Re-entry Contract $\Psi(s_t)$.
%     \item \textbf{Toolset Expansion ($\mathcal{T}_{merged}$)}: The Heterogeneous Toolset $\mathcal{T}_{merged}$ is expanded to include not only tuned existing operators but also \textbf{newly synthesized tools}. These executable scripts encapsulate specialized physical skills (e.g., high-precision impedance control) generated during the repair phase to address constraints beyond the base VLA's capabilities.
% \end{itemize}
% Mathematically, this consolidation operator is defined as:
% \begin{equation}
%     \mathcal{H}_{merged} = \text{Consolidate} \left( \{ \mathcal{H}_{patch, j} \mid seed_j \in K_i \} \right)
% \end{equation}

% \paragraph{Harness Packaging and Portability}
% To ensure the portability and version control of the evolved capabilities, $\mathcal{A}_{gen}$ encapsulates $\mathcal{H}_{merged}$ into a standardized, self-contained file structure. This package externalizes the governance logic from the agent code, mapping components to distinct directories:
% \begin{itemize}
%     \item \textbf{$SKILL.md$}: Declares the high-level governance logic, including defined milestones $M$, Orchestrator adjudication rules, and the generalized re-entry predicate $\Psi(s_t)$.
%     \item \textbf{$tools/$}: Contains the executable implementations and scripts for the evolved critics $C_{merged}$ and the toolset $\mathcal{T}_{merged}$.
%     \item \textbf{$plans/$}: Stores the generalized recovery playbooks $R_{merged}$, mapping specific evidence to structured intervention strategies.
%     \item \textbf{$params/$}: Holds the configuration files defining generalized numeric boundaries and thresholds for runtime execution.
% \end{itemize}

% \paragraph{Rigorous Generalization Validation}
% The final validated harness $\mathcal{H}_{merged}$ must satisfy stringent performance criteria via a dual-evaluation protocol. First, it must undergo **Historical Regression** testing, successfully resolving all failed rollouts within the originating cluster $K_i$ with a 100\% success rate:
% \begin{equation}
%     \forall seed_j \in K_i, \text{Success}(seed_j \mid \mathcal{H}_{merged}) = 1
% \end{equation}
% Second, to confirm genuine generalization, the harness is subjected to **Held-out Evaluation** on a strictly isolated dataset $\mathcal{D}_{held-out}$. The effectiveness of the evolution is quantified by the success rate increment $\Delta SR$ over the baseline VLA policy:
% \begin{equation}
%     \Delta SR = SR(\mathcal{D}_{held-out} \mid \mathcal{H}_{merged}) - SR(\mathcal{D}_{held-out} \mid \pi_{VLA})
% \end{equation}
% An evolutionary iteration is considered complete only when $\mathcal{H}_{merged}$ demonstrates robust performance on previously unseen data. If $\mathcal{D}_{held-out}$ reveals novel failure mechanisms requiring harness modification, the system triggers the \textbf{Dynamic Transition Protocol}, reclassifying the seed and initiating a new cycle.


% \subsection{Phase III: Harness Generalization, Consolidation, and Harness Packaging ($\mathcal{A}_{gen}$)}

% In the final stage of the evolutionary cycle, the system transitions from seed-specific local patches to the construction of mechanism-level harness. This phase is led by the Generalization Agent $\mathcal{A}_{gen}$, whose objective is to integrate and optimize all local patches $\mathcal{H}_{patch, j}$ validated in Stage 2 into a robust, versioned \textbf{merged harness $\mathcal{H}_{merged}$}.

% \subsubsection{Repair Abstraction and Consolidation}
% $\mathcal{A}_{gen}$ identifies \textbf{task invariants} by comparing Stage-2 repairs across diverse seeds to eliminate overfitting. The objective is to find a minimal governance configuration $\mathcal{H}_{merged}$ capable of repairing all historical failure samples within the same cluster $K_i$. We define the consolidation operator as follows:
% \begin{equation}
%     \mathcal{H}_{merged} = \text{Consolidate} \left( \{ \mathcal{H}_{patch, j} \mid seed_j \in K_i \} \right)
% \end{equation}
% where the construction of $\mathcal{H}_{merged} = \{C_{merged}, R_{merged}, \mathcal{T}_{merged}\}$ follows:
% \begin{itemize}
%     \item \textbf{Critic Unification ($C_{merged}$)}: Multiple local critics $C^*$ addressing the same failure mechanism are merged. By applying logical OR operations on triggering conditions and decorrelating parameters, $C_{merged}$ ensures stable proposal $P_t$ generation across varying initial distributions.
%     \item \textbf{Playbook Integration ($R_{merged}$)}: Local recovery playbooks $R^*$ are abstracted into generalized strategies. The merged playbook must handle multiple variations of the same failure mechanism and unify the re-entry contract $\Psi(s_t)$.
%     \item \textbf{Toolset Expansion and Adaptation ($\mathcal{T}_{merged}$)}: This is the core of the system's evolving executive capability. $\mathcal{T}_{merged}$ includes not only existing operators with tuned parameters but also \textbf{new specialized tools} introduced during the repair phase. These new tools are execution scripts implemented to address specific physical constraints (e.g., high-precision impedance control primitives) that the base VLA cannot cover.
% \end{itemize}

% \subsubsection{Harness Packaging and Component Mapping}
% To ensure the portability of governance capabilities, $\mathcal{A}_{gen}$ encapsulates the mathematically defined $\mathcal{H}_{merged}$ into a self-contained Harness package. This process establishes an explicit mapping between the file structure and the harness components:
% \begin{itemize}
%     \item \textbf{$SKILL.md$ (Governance Logic Declaration)}: Formally defines task milestones $M$, Orchestrator decision rules, and the re-entry predicate $\Psi(s_t)$. It serves as the top-level descriptor of $\mathcal{H}_{merged}$.
%     \item \textbf{$tools/$ (Implementation of Execution and Monitoring)}: Physically stores the code for runtime critics $C_{merged}$ and the scripts for the heterogeneous toolset $\mathcal{T}_{merged}$, including \textbf{newly synthesized tools}.
%     \item \textbf{$plans/$ (Strategy Playbook Collection)}: Stores the recovery playbooks $R_{merged}$ of $\mathcal{H}_{merged}$, containing mappings between failure evidence and action sequences.
%     \item \textbf{$params/$ (Parameter Configuration)}: Stores the generalized numeric boundaries, providing runtime configurations for $R_{merged}$ and $\mathcal{T}_{merged}$.
% \end{itemize}

% \subsubsection{Historical Regression and Held-out Generalization Protocol}
% Validation adheres to rigorous academic standards via a dual-set evaluation:
% \begin{enumerate}
%     \item \textbf{Historical Regression}: The merged harness $\mathcal{H}_{merged}$ must undergo closed-loop rollouts across all historical failure seeds. The pass criterion is:
%     \begin{equation}
%         \forall seed_j \in K_i, \text{Success}(seed_j \mid \mathcal{H}_{merged}) = 1
%     \end{equation}
%     \item \textbf{Held-out Evaluation}: The harness is evaluated on a strictly isolated set $\mathcal{D}_{held-out}$. Generalization efficacy is determined by the success rate increment $\Delta SR$ relative to the baseline VLA:
%     \begin{equation}
%         \Delta SR = SR(\mathcal{D}_{held-out} \mid \mathcal{H}_{merged}) - SR(\mathcal{D}_{held-out} \mid \pi_{VLA})
%     \end{equation}
% \end{enumerate}

% \subsubsection{Dynamic Transition Protocol}
% To maintain statistical integrity, the system enforces a strict \textbf{Dynamic Transition Protocol}. If a new failure mechanism is discovered in $\mathcal{D}_{held-out}$ and triggers modifications to $\mathcal{H}_{merged}$, the sets are updated:
% \begin{equation}
%     \mathcal{D}_{dev} \leftarrow \mathcal{D}_{dev} \cup \{seed_{failed}\}, \quad \mathcal{D}_{held-out} \leftarrow \mathcal{D}_{held-out} \setminus \{seed_{failed}\}
% \end{equation}
% The original held-out seed is reclassified as a development seed, and a fresh, previously unseen set must be selected for final validation. An evolutionary iteration is complete only when the harness passes a fresh test set without targeted adjustments.























\section{Z-Infra: Embodied Agent Rollout Infrastructure}

\subsection{Overview}

The rollout infrastructure serves as the execution backbone for the self-evolving embodied agent described above.
Its primary responsibility is to efficiently execute large-scale parallel rollouts (complete episodes of agent-environment interaction) across heterogeneous compute resources while exposing a simple, unified interface to upper-layer agent logic.

A single rollout proceeds as follows.
The agent first requests a \emph{session}, which provisions an isolated environment instance on an appropriate simulation environment, and then issues a \texttt{reset} call to initialize an episode.
The main execution loop iterates: the agent observes the environment state and invokes \texttt{policy\_step} to query a policy model for actions, or calls perception models and primitive operations as needed.
This loop continues until termination (success, failure, or timeout), at which point the session is released.


The self-evolving agent runs \emph{many such rollouts concurrently}, exploring different tasks, testing learned skills, and collecting experience for reflection, making efficient multiplexing of shared compute resources essential.
Although this work primarily considers the CPU-centric MuJoCo~\cite{todorov2012mujoco}/robosuite~\cite{zhu2020robosuite} stack used by LIBERO~\cite{liu2023libero} and RoboCasa~\cite{nasiriany2024robocasa}, embodied simulation also includes GPU-parallel MuJoCo backends such as MJX~\cite{mujocoteam2026mjx} and MJLab~\cite{zakka2026mjlab}, as well as PhysX-based stacks such as SAPIEN/ManiSkill~\cite{xiang2020sapien,gu2023maniskill2} and Isaac Sim/Isaac Lab~\cite{gao2026nvidia,mittal2025isaac}.
The rollout interface is designed to accommodate these backend differences while presenting the same session-level interaction model to the agent.

\subsection{Challenges and Key Ideas}

The agentic rollout workload described above poses two fundamental infrastructure challenges:

\paragraph{Resource Heterogeneity.}
A single rollout simultaneously demands diverse compute resources.
For the CPU-centric simulations, MuJoCo/robosuite environments maintain per-session simulation state and consume host CPU and memory during environment stepping, while their conventional rendering pipelines commonly use GPUs.
GPU-parallel simulation backends instead advance batches of environments on accelerators, with different requirements for state layout, reset semantics, rendering, and device memory.
Policy models require GPU accelerators for autoregressive or diffusion-based action generation and GPU memory to store computing feature~\cite{li2026oxygen,xu2026embodied,ma2025runningvlasrealtimespeed,tang2025vlash}.
Lightweight perception models~\cite{carion2025sam3segmentconcepts,kirillov2023segment,Jocher_Ultralytics_YOLO26_Unified_2026,redmon2016you,ding2025streammind,zheng2026emgardeproposematchframeworkproactive,fang2023robust,sundermeyer2021contact} can share GPU resources but have distinct latency requirements.
Primitive operations (coordinate transforms, collision checks) are pure CPU computations with microsecond-scale latency expectations.
These workloads lead to different worker and scheduling requirements, so no single resource pool or scheduling policy fits all these workload types.

\paragraph{Execution Dynamism.}
Unlike training pipelines with predictable data-parallel patterns, agentic rollouts exhibit inherently unpredictable execution profiles.
The agent dynamically selects which tools to invoke based on runtime observations, one timestep may require only a policy call, while the next may chain perception, planning, and multiple primitive operations.
Sessions are created, paused, and destroyed at irregular intervals as the agent explores tasks, reflects on failures, and retries with modified strategies.
This results in bursty GPU inference demands with high variance in batch sizes and inter-arrival times, making static resource allocation and request scheduling inefficient.

\paragraph{Key Idea: Decoupled Abstraction Layers.}
We address these challenges by introducing an abstraction layer that fully decouples agent logic from hardware resource management.
The agent interacts exclusively with a virtual rollout interface---specifying \emph{what} to execute (which model, which environment, which operation) without concern for \emph{where} or \emph{how} execution occurs.
The infrastructure independently handles worker allocation, request routing, batch formation, and hardware mapping, enabling transparent scaling across multi-node, multi-GPU clusters without requiring changes to agent code.
This separation of concerns allows each layer to be optimized independently: agent developers focus on task logic and skill composition, while infrastructure engineers optimize scheduling, batching, and hardware utilization.

\subsection{System Architecture}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.72\linewidth]{figs/infra_arch_v2.pdf}
  \caption{Three-layer architecture of the rollout infrastructure. The Control Plane routes agent requests to specialized Env Workers and Rollout Workers, which manage environment simulation and model inference respectively.}
  \label{fig:infra-architecture}
\end{figure}

The infrastructure is organized into three layers (Figure~\ref{fig:infra-architecture}), each addressing a distinct concern in the execution pipeline.
The \textbf{Control Plane} serves as the single entry point for all agent interactions, exposing a unified API that abstracts over backend heterogeneity and handles request routing, resource management, and fault tolerance.
The \textbf{Environment Worker Layer} manages the lifecycle and execution of simulation environments across diverse families, handling session provisioning, environment stepping, and observation capture.
The \textbf{Rollout Worker Layer} provides GPU-resident model serving for VLA/WAM policies and perception models, implementing batched inference with dynamic scheduling to maximize throughput under variable request patterns.
These layers communicate via bounded asynchronous channels that enforce backpressure and enable transparent scaling across multi-node GPU clusters.

\subsubsection{Control Plane}

The Control Plane serves as the infrastructure's coordination hub, decoupling agent logic from distributed resource management.
It exposes a unified API that routes each request to the appropriate worker pool based on request type (environment operation vs. model inference) and resource requirements (environment family, model type).
The Gateway maintains a global session registry that tracks the binding between sessions and Env Worker ranks, enabling efficient request dispatch without requiring agents to manage worker topology.
Worker health is monitored via periodic heartbeats: when an Env Worker fails, the Gateway detects the timeout, marks affected sessions as \texttt{LOST}, and returns failure notifications to agents, which can then recreate sessions on healthy workers.

% Admission control is enforced at two levels: session-level lease mechanisms prevent resource leaks from abandoned sessions by requiring periodic renewal, while request-level backpressure rejects new operations when downstream queues are saturated.
% The Gateway also performs load balancing: environment operations are dispatched to Env Workers with available slots, prioritizing workers with lighter session loads, while inference requests are forwarded to the shared request channel where Rollout Workers compete for work.

\subsubsection{Environment Worker}

The Environment Worker layer addresses the challenge of managing heterogeneous simulation environments at scale while maintaining session isolation and maximizing resource utilization.
Each Env Worker is a distributed actor that hosts multiple environment slots, where each slot binds to an active session and maintains its own execution state.
The layer must support diverse environment families with different APIs (reset signatures, observation structures, action formats) and execution models (CPU subprocesses vs. GPU-batched simulation), while exposing a uniform interface to the Control Plane.

\paragraph{Session-based Lifecycle Management.}
We introduce a session abstraction to support long-lived agent-environment interactions.
Each session encapsulates an independent execution context, binding to a specific environment slot on an Env Worker and progressing through a well-defined lifecycle: \texttt{CREATE} $\rightarrow$ \texttt{RUNNING} $\rightarrow$ \texttt{TERMINATED}.
Upon creation, the Gateway selects an appropriate Env Worker based on resource availability and environment family compatibility, allocates a slot, and returns a session handle to the agent.

The session registry maintained by the Gateway enables efficient resource accounting and admission control.
At any point, the system knows exactly how many sessions of each environment family are active, their distribution across workers, and remaining lease durations.
When workers are saturated, new session requests are rejected with backpressure signals, preventing cascading overload.

To onboard new environment families, developers implement four primitives through a declarative registration framework:
\textbf{(i)} \texttt{init}---construct the environment from a configuration dictionary;
\textbf{(ii)} \texttt{reset}---reset to an initial state given task-specific parameters;
\textbf{(iii)} \texttt{step}---execute an action and return observation, reward, and termination flags;
\textbf{(iv)} \texttt{obs\_schema}---declare the structure and encoding of observations.
A normalization layer translates family-specific observations into a canonical format (dictionaries of named tensors with declared shapes and dtypes), ensuring that upper-layer code remains family-agnostic.

\paragraph{Resource-Sharing Group.}
For parallel benchmark rollouts using MuJoCo-based environments (e.g., LIBERO~\cite{liu2023libero}, RoboCasa~\cite{nasiriany2024robocasa}), we implement a resource-sharing optimization that amortizes model compilation and rendering context setup across multiple sessions.
The resource-sharing group is the execution unit for sessions with identical environment structure and configuration.
The group compiles the environment model once into a \texttt{ModelTemplate}, which retains the reusable read-only \texttt{mjModel} representation together with the initial simulation state.
Each slot is initialized through a fork primitive from this template, allowing the group to reuse immutable model resources while each slot maintains its own \texttt{mjData} and episode state.
This separates shared model structure from mutable simulation state: resetting or stepping one slot does not modify the state of any other slot in the group.

The group also owns the execution resources required by the slots.
Each slot is assigned to a pinned worker thread with a thread-local render context, while the contexts belong to a shared render context group, allowing compatible GPU rendering resources to be reused across slots without cross-thread context conflicts.
To make this resource sharing effective under multithreaded execution, the environment step routine is reimplemented with a high-performance C++ controller that combines control execution, action interpolation, physics substeps, and rendering, while minimizing Python-side overhead.
With the GIL released during the critical path, multiple slots advance their physics and rendering workloads in parallel within the same worker process.

\subsubsection{Rollout Worker}

The Rollout Worker layer addresses the challenge of serving diverse neural models under dynamic, bursty request patterns while maximizing GPU utilization.
Each Rollout Worker is a GPU-resident actor that executes batched inference and returns results asynchronously.
Workers are organized into specialized pools: policy models occupy dedicated high-memory GPUs, while lightweight perception models are co-located on shared GPUs.
The layer must balance throughput (larger batches amortize GPU kernel overhead) against latency (requests should not wait indefinitely), while handling compatibility constraints (only requests with matching model type, input modalities, and tensor shapes can be batched together).

\paragraph{Scheduler.}
The Rollout Worker Scheduler manages the full lifecycle of inference requests from arrival to result delivery across a pool of GPU-resident workers.
Upon receiving an inference request, the scheduler first classifies it into a compatibility group based on model identity, input modalities, and tensor shapes, then enqueues it into the corresponding per-group request queue.
The scheduler monitors worker load and dispatches batched requests to available workers in a first-come-first-served (FCFS) manner to ensure high overall resource utilization while maintaining low per-request latency.
When a Rollout Worker completes a batch, it tags each result with its routing token and publishes it to a shared result channel; the originating Env Worker retrieves its results by token match, enabling fully asynchronous request-response patterns without blocking.

\paragraph{Model Partitioning.}
Modern VLA/WAM architectures (e.g., $\pi_{0.5}$~\cite{black2025pi05}) consist of two functionally distinct stages: a Vision-Language Model (VLM) that encodes observations and instructions into latent representations, and an Action Expert (AE) that decodes these representations into motor commands via diffusion or autoregressive generation.
These stages have markedly different computational characteristics.
We exploit these different characteristics by deploying the VLM and AE as separate processes with independent scheduling policies.
VLM's intermediate activations are transferred between VLM and AE processes via CUDA IPC to avoid expensive transmission overhead.
For the $\pi_{0.5}$ model implemented in PyTorch, this partitioning strategy reduces average inference latency by 53\% and improves goodput (under 200ms SLO) by 2.4$\times$ compared to monolithic deployment.

\paragraph{Quantization Runtime.}
To improve policy inference throughput and GPU memory efficiency, we introduce quantization (e.g., W8A8, W4A16, W4A8) as an \emph{optional} plug-in to the Rollout Worker.
Unlike model-level quantization in common LLM serving frameworks~\cite{kwon2023efficient,zheng2024sglang}, we quantize different modules inside a policy model separately, co-designed with model partitioning, as well as to balance policy success rates and inference efficiency. For $\pi_{0.5}$ on RTX 4090, we currently apply W8A8 quantization for the  compute-intensive prefix MLP modules, while keeping other modules at BF16 to avoid additional overhead, achieving $1.18\times$--$1.32\times$ inference speedup without degrading success rates on LIBERO.

\subsubsection{Implementation.}
The infrastructure is built on Ray~\cite{222605} for distributed execution.
Each Env Worker and Rollout Worker is a Ray actor wrapping the respective runtime logic, with resource annotations declared via placement strategies.
We use Ray's placement strategy to bind each worker to a dedicated GPU/CPU.
For example, declaring \texttt{placement: "0-7"} provisions 8 ranks, each mapped to one GPU (e.g., 8 A100s on a single node, or distributed across nodes in multi-node setups).
Each rollout rank loads an independent copy of the model, enabling data-parallel inference across the rank pool.

Communication across the three layers is structured around five bounded Ray Channels that partition control flow and data flow.
Command and control channels route lifecycle operations and priority signals from Gateway to Env Workers, while result channels return step outcomes in the reverse direction.
Inference requests flow from Env Workers to a shared channel consumed competitively by all Rollout Workers, enabling load-aware distribution; responses are routed back via embedded tokens.


\subsection{Programming Support}

The infrastructure exposes a layered programming model designed to minimize cognitive overhead for agent developers while retaining full flexibility for advanced use cases.
The model is organized around three core abstractions: \textbf{sessions} represent long-lived environment instances with managed lifecycles, \textbf{episodes} run within sessions from reset to termination, and \textbf{steps} execute individual actions within episodes.
Agents interact through a clean API that handles batching, asynchronous inference, and resource management transparently---developers specify \emph{what} they want (e.g., ``execute this policy in these environments''), and the infrastructure determines \emph{how} to schedule workers, batch requests, and route results efficiently.

\paragraph{API Overview.}
Table~\ref{tab:api-primitives} summarizes the core API exposed to upper-layer agents, organized into five categories: \textit{Session Management} handles environment lifecycle (create, renew, close); \textit{Observation \& State} provides environment introspection; \textit{Low-Level Control} executes motor commands (Cartesian servoing, gripper control); \textit{Policy Execution} integrates model serving (\texttt{policy\_step} for atomic observe-infer-step operations, \texttt{run\_episode} for autonomous execution); and \textit{Perception \& Planning} provides high-level services (segmentation, grasp generation, motion planning).
All APIs support transparent batching across multiple sessions.

\begin{table}[t]
\centering
\small
\begin{tabular}{@{}p{0.38\linewidth}p{0.58\linewidth}@{}}
\toprule
\textbf{API Primitive} & \textbf{Functionality} \\
\midrule
\multicolumn{2}{@{}l}{\textit{Session Management --- create once, run many episodes, close when done}} \\
\texttt{create\_sessions(requests)} & Batch create sessions with env\_family, env\_config, lease\_seconds. Returns SessionHandle with session\_id. \\
\texttt{renew\_sessions(session\_ids)} & Extend lease duration for active sessions. \\
\texttt{close\_sessions(session\_ids)} & Close sessions and release resources (idempotent). \\
\midrule
\multicolumn{2}{@{}l}{\textit{Environment Control --- direct interaction for custom control logic}} \\
\texttt{reset(session\_ids, reset\_spec)} & Start new episode with task\_id, seed, instruction. Returns episode\_id and initial observation. \\
\texttt{observe(session\_ids)} & Read current observation without side effects. \\
\texttt{action\_step(session\_ids, actions)} & Execute actions, return observation, reward, terminated, truncated flags. \\
\midrule
\multicolumn{2}{@{}l}{\textit{Policy Inference --- integrated model serving and stepping}} \\
\texttt{policy\_step(session\_ids, policy\_req)} & Atomic observe $\rightarrow$ inference $\rightarrow$ step. Returns step results with executed actions. \\
\texttt{policy\_infer(session\_ids, policy\_req)} & Inference only (no stepping). Returns actions for agent post-processing. \\
\texttt{run\_episode(session\_ids, episode\_req)} & Execute complete episodes in workers. Returns summary (steps, reward, stop\_reason). \\
\bottomrule
\end{tabular}
\caption{Core API primitives exposed to agents. All primitives support batching across sessions.}
\label{tab:api-primitives}
\end{table}

\begin{lstlisting}[language=Python, style=rolloutflow, caption={Simplified pseudocode for a \texttt{policy\_step} call spanning the Agent, Gateway, EnvWorker, and RolloutWorker layers.}, label=lst:execution-flow, captionpos=b, float, floatplacement=t]
# === Agent Side ===
sessions = await gateway.create_sessions(env_family="maniskill", n=16)
obs = await sessions.reset(task_id="pick_cube")
for _ in range(max_steps):
    result = await sessions.policy_step(instruction="pick_up_the_red_cube")
await sessions.close()

# === Gateway: policy_step dispatch ===
async def policy_step(session_id, instruction):
    worker_rank = registry.get_worker(session_id)
    return await send_command(worker_rank, "POLICY_STEP",
                               session_id=session_id, instruction=instruction)

# === EnvWorker: handle policy_step ===
async def handle_policy_step(session_id, instruction):
    token = make_routing_token(self.rank, session_id)
    await infer_req_ch.put(observation=session.obs, instruction=instruction,
                           routing_token=token)       # non-blocking, yield
    action = await infer_resp_ch.get(key=token)       # wake on response
    outcome = env.step(action)
    return StepResult(outcome)

# === RolloutWorker: batched inference ===
async def serve():
    while True:
        batch = await scheduler.next_batch()          # work-stealing
        actions = model.infer([r.obs for r in batch],
                              [r.inst for r in batch])
        for req, action in zip(batch, actions):
            await infer_resp_ch.put(key=req.routing_token, action=action)
\end{lstlisting}

\paragraph{Execution Flow.}
Listing~\ref{lst:execution-flow} illustrates a \texttt{policy\_step} call across the three infrastructure layers.
From the agent's perspective, the interaction is simple: create a session, reset the episode, and loop over \texttt{policy\_step}.
Internally, the Gateway routes each step to the session's Env Worker, which packages an inference request with a routing token and submits it to the shared channel before yielding to serve other sessions.
A Rollout Worker pulls the request, executes batched inference, and routes the result back via the token.
The Env Worker then steps the environment and returns the outcome, completing the pipeline while other sessions on the same worker continue making progress.


==> arxiv_submission/tex/packages_macros.tex <==
% !TEX root = ../neurips_2026.tex
% packages
% \usepackage{microtype}
\usepackage{xspace}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{multirow}
% \usepackage{subfigure}
\usepackage{makecell}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{enumitem}

% \usepackage{ulem}
\usepackage[ruled,linesnumbered,noend]{algorithm2e}
% \usepackage{algpseudocode}
\usepackage{hyperref}
% \usepackage{tcolorbox}
\usepackage{listings}
\lstdefinestyle{rolloutflow}{
  basicstyle=\ttfamily\small,
  backgroundcolor=\color{gray!10},
  frame=single,
  framerule=0.4pt,
  rulecolor=\color{gray!50},
  breaklines=true,
  columns=fullflexible,
  keepspaces=true,
  commentstyle=\color[RGB]{0,128,0},
  morecomment=[l]{\#}
}
% \lstset{
%   basicstyle=\ttfamily\small,
%   backgroundcolor=\color{gray!10},
%   frame=single,
%   framerule=0.4pt,
%   rulecolor=\color{gray!50},
%   breaklines=true,
%   columns=fullflexible,
%   keepspaces=true,
%   commentstyle=\color[RGB]{0,128,0},  % green for # comments
%   morecomment=[l]{\#},
% }

% macros
\newcommand{\sys}{Zetta\xspace}
% \newcommand{\reponame}{\texttt{vlut.cpp}\xspace}
% \newcommand{\codelink}{\url{https://github.com/OpenBitSys/vlut.cpp}\xspace}

\newcommand{\xiangyu}[1]{{\color{blue}{[xiangyu: #1]}}\xspace}
\newcommand{\yunxin}[1]{{\color{red}{[yunxin: #1]}}}
\newcommand{\bingjia}[1]{{\color{orange}{[bingjia: #1]}}\xspace}
\newcommand{\ting}[1]{{\color{brown}{[ting: #1]}}\xspace}
\newcommand{\mi}[1]{{\color{purple}{[mi: #1]}}\xspace}
\newcommand{\haozx}[1]{{\color{teal}{[haozx: #1]}}\xspace}


==> arxiv_submission/tex/related.tex <==
\section{Related Work}
We organize related work around the motivation for closed-loop embodied learning. First, physical intelligence is scaling through both foundation models and agent harnesses, but the deployment gap remains. Second, self-evolving agents have shown strong progress in digital domains, yet embodied self-evolution is harder because the agent must interpret and act in a continuous physical world. Third, existing rollout systems are mostly designed for standard RL workloads, while embodied self-evolution requires heterogeneous model, tool, simulator, robot, memory, and critic execution.

\subsection{Embodied Foundation Model Gaps for Physical Intelligence Scaling}
Recent physical intelligence research is advancing along two complementary paths. The first path trains end-to-end policy models for general robot control, including VLA models such as RT-1/RT-2, OpenVLA, $\pi_0$, $\pi_{0.5}$, GR00T, CogACT, UniVLA, and FAST, as well as world-action models such as DreamZero, Cosmos-Policy, and FAST-WAM \citep{brohan2022rt1,brohan2023rt2,kim2024openvla,black2024pi0,black2025pi05,bjorck2025groot,li2024cogact,bu2025univla,pertsch2025fast,dreamzero2026,cosmospolicy2026,fastwam2026}. This line is promising, but real deployment still exposes a \textbf{persistent gap}: data are expensive, physical distributions shift, and small execution errors can cascade in long-horizon tasks, which limits end-to-end models from moving beyond demonstrations into real-world productivity. 

The second path explores embodied agent capabilities by using LLMs, code, tools, memory, planning, verification, and recovery around foundation policies to fill this gap. Earlier systems such as PaLM-E and Code as Policies demonstrated the potential of language models for embodied reasoning and planning, while RoboCat showed that an agent can broaden its manipulation competence by collecting data from its own attempts across tasks and embodiments \citep{driess2023palme,liang2023codeaspolicies,bousmalis2023robocat}. Recent systems and demonstrations, including Claude Plays Robotics, CaP-X, HarnessVLA, and Guava, further suggest that coding agents and execution scaffolds can make frozen or pretrained robot policies more reliable without waiting for a fully solved end-to-end policy \citep{anthropic2026clauderobotics,capx2026,zhang2026harnessvla,liu2026guava}. The state of the art is therefore shifting from relying only on a single end-to-end policy toward scaffolded systems that coordinate policies with planning, memory, tools, verification, and recovery. 

However, many embodied agents remain episodic: they may recover within a trial, but they rarely convert execution traces into governed long-term improvements. Our work follows the embodied-agent path by studying a closed-loop harness that turns deployment feedback into reusable critics, recoveries, and future rollouts.

\subsection{Live Harness Gaps for Embodied Self-Evolution}
General agent self-evolution has mainly been studied in digital domains where execution is cheap, interfaces are discrete, APIs are explicit, logs are exact, and evaluation is relatively easy. Reflexion, Self-Refine, Voyager, and OPRO show that language or game agents can improve through verbal feedback, iterative revision, executable skill libraries, or search over prompts and programs \citep{shinn2023reflexion,madaan2023selfrefine,wang2023voyager,yang2024opro}. Recent surveys summarize this loop as generation, execution, evaluation, reflection, memory update, and sometimes model or prompt optimization \citep{gao2025selfevolvingagents,ren2026selfimprovingagents, ding2026memcompiler}. 

Embodied agents face a harder version of this problem because they operate in a continuous world: the harness must evaluate both robot state and world state, decide when to call policies, tools, critics, or recovery modules, and prevent early errors from becoming hard-to-recover physical failures. Moreover, current VLAs are far weaker and less reliable than frontier LLMs in their native digital domains, so embodied agents need more external tools, verifiers, memories, and frequent critics to support robust execution. Real-world policy-improvement systems such as ENPIRE, Visual Verification/VERITAS, Learning While Deploying, and SOP show that robot deployment can be organized as a closed loop of execution, verification, data selection, and policy update rather than a one-time training pipeline \citep{xiao2026enpire,li2025veritas,agibot2026lwd,agibot2026sop}. Skill-centric systems such as ASPIRE, ReSYNC, VASO, and EmbodiSkill instead emphasize discovering reusable programs, concepts, contracts, or skills from failures and reflections \citep{aspire2026,zhang2026resync,vaso2026formal,embodiskill2026}. Test-time and reasoning-oriented systems such as RoboTTT, R\&B-EnCoRe, EEAgent, and SEEA-R1 further show that adaptation can happen through long context, richer feedback, reflection, or reinforcement tuning \citep{robottt2026,renbencore2026,wang2026eeagent,seea2025,ding2025adanav}. 

Existing systems usually improve one layer of the stack, such as code, prompts, verifiers, memories, or policy data, but few jointly address high-frequency runtime critics, recoverable failure traces, reusable recovery skills, and high-throughput rollout execution. Our design targets this combined gap by grounding reflection in runtime critics and recovery actions, then using rollout infrastructure to repeatedly evaluate, replay, and improve embodied agents.

\subsection{Rollout Infrastructure Gaps for Embodied Self-Evolution}
There is still little infrastructure work designed specifically for self-evolving embodied agents. Most mature rollout systems come from general RL or distributed learning, such as A3C-style asynchronous actors, IMPALA, SEED RL, RLlib/Ray, Acme, and recent large-scale RL systems such as RLinf \citep{mnih2016a3c,espeholt2018impala,espeholt2020seed,liang2018rllib,hoffman2020acme,yu2025rlinf}. These systems established important ideas such as actor-learner separation, scalable experience collection, centralized inference, and flexible execution graphs. 

However, \textbf{embodied rollouts add workloads that are not central in standard rollout runtimes}: VLA inference, diffusion or flow action heads, perception encoders, tool calls, memory retrieval, simulators, real robot workers, resets, safety checks, and verifier/critic models. As a result, throughput is limited not only by environment stepping, but also by heterogeneous model serving and coordination across CPU, GPU, robot, and cloud resources. Another bottleneck is extensibility: adding a new simulator, tool, model backend, or agent variant often requires changing orchestration code instead of registering a new component behind a stable interface. These limits directly slow self-evolution because fewer failures can be discovered, diagnosed, replayed, and converted into reusable improvements per unit time. Our rollout infrastructure is designed for this embodied workload mix through decoupled execution, continuous batching, resource-sharing environments, and fine-grained processor control.

